Stellar Diameters and Temperatures II. Main Sequence K & M Stars

We present interferometric diameter measurements of 21 K- and M- dwarfs made with the CHARA Array. This sample is enhanced by literature radii measurements to form a data set of 33 K-M dwarfs with diameters measured to better than 5%. For all 33 stars, we compute absolute luminosities, linear radii, and effective temperatures (Teff). We develop empirical relations for \simK0 to M4 main- sequence stars between the stellar Teff, radius, and luminosity to broad-band color indices and metallicity. These relations are valid for metallicities between [Fe/H] = -0.5 and +0.1 dex, and are accurate to ~2%, ~5%, and ~4% for Teff, radius, and luminosity, respectively. Our results show that it is necessary to use metallicity dependent transformations to convert colors into stellar Teffs, radii, and luminosities. We find no sensitivity to metallicity on relations between global stellar properties, e.g., Teff-radius and Teff-luminosity. Robust examinations of single star Teffs and radii compared to evolutionary model predictions on the luminosity-Teff and luminosity-radius planes reveals that models overestimate the Teffs of stars with Teff < 5000 K by ~3%, and underestimate the radii of stars with radii < 0.7 R\odot by ~5%. These conclusions additionally suggest that the models overestimate the effects that the stellar metallicity may have on the astrophysical properties of an object. By comparing the interferometrically measured radii for single stars to those of eclipsing binaries, we find that single and binary star radii are consistent. However, the literature Teffs for binary stars are systematically lower compared to Teffs of single stars by ~ 200 to 300 K. Lastly, we present a empirically determined HR diagram for a total of 74 nearby, main-sequence, A- to M-type stars, and define regions of habitability for the potential existence of sub-stellar mass companions in each system. [abridged]

==> Ref_Object_phot_forfits.tex <==
%\begin{landscape}

\begin{deluxetable}{lcccccccc}
\tabletypesize{\tiny}
\tablewidth{0pt}
%\tablenum{1}
\tablecaption{Object Photometry used in Relations \label{tab:Ref_Object_phot_forfits}}
\tablehead{
\colhead{\textbf{ }} &
\colhead{\textbf{$B$}} &
\colhead{\textbf{$V$}} &
\colhead{\textbf{$R$}} &
\colhead{\textbf{$I$}} &
\colhead{\textbf{$J$}} &
\colhead{\textbf{$H$}} &
\colhead{\textbf{$K$}} &
\colhead{\textbf{Reference$_{BVRI}$,}} \\
\colhead{\textbf{Star}} &
\colhead{\textbf{(mag)}} &
\colhead{\textbf{(mag)}} &
\colhead{\textbf{(mag)}} &
\colhead{\textbf{(mag)}} &
\colhead{\textbf{(mag)}} &
\colhead{\textbf{(mag)}} &
\colhead{\textbf{(mag)}} &
\colhead{\textbf{Reference$_{JHK}$}}
}
\startdata

GJ 15 A	\dotfill &	9.63	&	8.07	&	6.69	&	5.53	&	4.86	&	4.25	&	4.02	&  \citet{1965ApJ...141..170J,1975MNRAS.171P..19G}	\\
%GJ 33	\dotfill &	6.64	&	5.76	&	4.99	&	4.52	&	4.24	&	3.72	&	3.61	&  \citet{1966CoLPL...4...99J,1968ApJ...152..465J}	\\
GJ 53 A	\dotfill &	5.87	&	5.18	&	4.55	&	4.14	&	3.86	&	3.39	&	3.36	&  \citet{1966CoLPL...4...99J,1968ApJ...152..465J}	\\
GJ 75	\dotfill &	6.44	&	5.63	&	4.99	&	4.60	&	4.31	&	3.88	&	3.84	&  \citet{1966CoLPL...4...99J,1989AA...215..305A}	\\
%GJ 105 A	\dotfill &	6.79	&	5.82	&	4.99	&	4.46	&	4.07	&	3.52	&	3.45	&  \citet{1966CoLPL...4...99J,1975MNRAS.171P..19G}	\\
GJ 144	\dotfill &	4.62	&	3.74	&	3.01	&	2.55	&	2.20	&	1.75	&	1.65	&  \citet{1966CoLPL...4...99J,1975MNRAS.171P..19G}	\\
GJ 166 A	\dotfill &	5.25	&	4.43	&	3.74	&	3.29	&	2.95	&	2.48	&	2.41	&  \citet{1966CoLPL...4...99J,1968ApJ...152..465J}	\\
%GJ 205	\dotfill &	9.44	&	7.97	&	6.53	&	5.39	&	4.77	&	4.06	&	3.86	&  \citet{1965ApJ...141..170J,1976ApJ...208..399M}	\\
GJ 380	\dotfill &	7.94	&	6.59	&	5.36	&	4.56	&	3.98	&	3.32	&	3.19	&  \citet{1965ApJ...141..170J,1975MNRAS.171P..19G}	\\
GJ 411	\dotfill &	9.00	&	7.49	&	5.99	&	4.80	&	4.13	&	3.56	&	3.35	&  \citet{1964BOTT....3..305J,1975MNRAS.171P..19G}	\\
GJ 436	\dotfill &	12.17	&	10.65	&	100.00	&	100.00	&	6.90	&	6.32	&	6.07	&  \citet{1993AJ....105.1962W,2003yCat.2246....0C}	\\
%GJ 514	\dotfill &	10.55	&	9.06	&	7.61	&	6.52	&	6.02	&	5.31	&	5.10	&  \citet{1965ApJ...141..170J,1971BITon...6..143E}	\\
%GJ 526	\dotfill &	9.93	&	8.50	&	7.06	&	5.92	&	5.26	&	4.64	&	4.46	&  \citet{1965ApJ...141..170J,1975MNRAS.171P..19G}	\\
%GJ 551	\dotfill &	13.02	&	11.05	&	8.68	&	6.42	&	5.33	&	4.73	&	4.37	&  \citet{1972PASP...84..581F,1976ApJ...208..399M}	\\
GJ 570 A	\dotfill &	6.88	&	5.78	&	4.85	&	4.28	&	3.82	&	3.27	&	3.15	&  \citet{1965ApJ...141..170J,1976ApJ...208..399M}	\\
GJ 581	\dotfill &	12.19	&	10.58	&	8.89	&	7.46	&	6.68	&	6.09	&	5.83	&  \citet{1965ApJ...141..170J,1976ApJ...208..399M}	\\
%GJ 631	\dotfill &	6.55	&	5.74	&	5.13	&	4.74	&	4.32	&	3.86	&	3.83	&  \citet{1966CoLPL...4...99J,1968ApJ...152..465J}	\\
%GJ 673	\dotfill &	8.89	&	7.53	&	6.23	&	5.43	&	4.97	&	4.28	&	4.14	&  \citet{1965ApJ...141..170J,1975MNRAS.171P..19G}	\\
%GJ 687	\dotfill &	10.62	&	9.17	&	100.00	&	100.00	&	5.37	&	4.75	&	4.54	&  \citet{1953ApJ...117..313J,1977AJ.....82..729P}	\\
GJ 699	\dotfill &	11.28	&	9.54	&	100.00	&	100.00	&	5.30	&	4.77	&	4.50	&  \citet{1997yCat.2168....0M,1976ApJ...208..399M}	\\
%GJ 752 A	\dotfill &	10.58	&	9.11	&	100.00	&	100.00	&	5.50	&	4.83	&	4.64	&  \citet{1953ApJ...117..313J,1975MNRAS.171P..19G}	\\
GJ 764	\dotfill &	5.49	&	4.69	&	4.04	&	3.63	&	3.32	&	3.04	&	2.78	&  \citet{1966CoLPL...4...99J,1966CoLPL...4...99J}	\\
GJ 820 A	\dotfill &	6.39	&	5.23	&	4.20	&	3.56	&	3.16	&	2.61	&	2.40	&  \citet{1966CoLPL...4...99J,1968ApJ...152..465J}	\\
GJ 820 B	\dotfill &	7.38	&	6.02	&	4.87	&	4.07	&	3.58	&	2.93	&	2.73	&  \citet{1966CoLPL...4...99J,1968ApJ...152..465J}	\\
GJ 845	\dotfill &	5.75	&	4.69	&	3.81	&	3.25	&	2.83	&	2.30	&	2.18	&  \citet{1966CoLPL...4...99J,1976ApJ...208..399M}	\\
%GJ 879	\dotfill &	7.59	&	6.49	&	5.54	&	4.95	&	4.53	&	3.80	&	3.81	&  \citet{1966CoLPL...4...99J,2003yCat.2246....0C}	\\
%GJ 880	\dotfill &	10.18	&	8.68	&	100.00	&	100.00	&	5.41	&	4.78	&	4.58	&  \citet{1971BITon...6..143E,1971BITon...6..143E}	\\
GJ 887	\dotfill &	8.83	&	7.35	&	100.00	&	100.00	&	4.20	&	3.60	&	3.36	&  \citet{1990AAS...83..357B,1976ApJ...208..399M}	\\

\enddata

%\tablenotetext{a}{Magnitude from 2MASS.}
\tablecomments{Refer to Section~\ref{sec:metallicities} for detials.}
\end{deluxetable}

%\end{landscape}




==> SED_phot.updated.tex <==

% this is a table from gerards two emails from 5-24-12 and 4-26 for object phot used in SED fits for Fbol determination

%%
%% Begining of file `table.tex'

%% This complex but short example prepared in the deluxetable environment
%% demonstrates some of the techniques
%% that can be used to generate complex column headings and to align
%% variable-width columns. See the manuscript sample file, sample.tex,
%% for more table examples.

%% Note this file has its own \documentclass, \begin{document}, and
%% \end{document} commands. If you want to insert this table in another
%% LaTeX document using the \input command, comment out these lines.

%----------
%comment these out for input into paper.

%\documentclass{aastex}

%\usepackage{natbib}
%\bibliographystyle{apj}

%\begin{document}
%----------

%% Note that the table will print double-spaced since we are using the
%% manuscript style. Change the style to preprint or preprint2 to see
%% how LaTeX formats the table in those styles.

%% In this example the LaTeX \multicolumn command is used to span a heading
%% over several columns.  When \multicolumn is used along with the
%% \cutinhead or \sidehead commands, the \tablecolumns command must
%% be used to specify the number of columns in the table -
%% otherwise \cutinhead and \sidehead will not work properly.

%% \cline has been used to produce straddle rules below the spanning heads,
%% \cutinhead to produce a centered head in the body of the table, and
%% \sidehead to produce a flush-left head in the body.

%% This table also makes use of the \phn command to better align some of the
%% columns.  Also see \phd, \phs, and \phm{} - other commands useful for
%% column alignment.  All of these commands insert a blank space
%% whose width is  equal to that of a number (\phn),
%% a decimal point (\phd), a minus sign (\phs), or any
%% character you wish to use (\phm{text}).
%% Keep in mind that if you are preparing a table for electronic submission
%% to one of the journals, you need not worry too much about column
%% alignment. The editors will fix table alignment as appropriate.

%% If a table is more than one page long, the width of the table can vary
%% from page to page when the default \tablewidth is used, as below.  The
%% individual table widths for each page will be written to the log file; a
%% maximum tablewidth for the table can be computed from these values.
%% The \tablewidth argument can then be reset and the file reprocessed, so
%% that the table is uniform throughout the pages. Try getting the widths
%% from the log file and changing the \tablewidth parameter to see how
%% adjusting this value affects table formatting.

%% The * option to the \\ command has been used in the lines after
%% the \sidehead to keep them together on the same page. Try taking
%% the *'s out and LaTeXing the manuscript again to see the difference
%% in the page breaks. You can group together as many lines as
%% you like using this command.											
											
											
\begin{deluxetable}{lccccl}											
\tablecolumns{6}											
\tabletypesize{\scriptsize}											
\tablewidth{0pc}											
%\tablecaption{More photometry than you could shake a stick at (again!)\label{tab:SED_phot}}											
\tablecaption{Object photometry used in SED fits \label{tab:SED_phot}}											
\tablehead{											
Star & System /  & Bandpass /  &  &  &  \\											
 ID &  Wavelength &  Bandwidth & Value & Error & Reference											
}											
\startdata											
GJ	15A	&	Stromgren	&	v	&	10.52	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	15A	&	Stromgren	&	v	&	10.52	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	15A	&	Stromgren	&	v	&	10.55	&	0.08	&	\citet{1974AJ.....79.1424O}\\
GJ	15A	&	Johnson	&	B	&	9.68	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	15A	&	Johnson	&	B	&	9.63	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	15A	&	Johnson	&	B	&	9.65	&	0.05	&	\citet{1974PASP...86..294U}\\
GJ	15A	&	Johnson	&	B	&	9.71	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	15A	&	Johnson	&	B	&	9.65	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	15A	&	Johnson	&	B	&	9.63	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	15A	&	Johnson	&	B	&	9.65	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	15A	&	Stromgren	&	b	&	9.04	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	15A	&	Stromgren	&	b	&	9.04	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	15A	&	Stromgren	&	b	&	9.12	&	0.08	&	\citet{1974AJ.....79.1424O}\\
GJ	15A	&	Stromgren	&	y	&	8.07	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	15A	&	Stromgren	&	y	&	8.07	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	15A	&	Stromgren	&	y	&	8.07	&	0.08	&	\citet{1974AJ.....79.1424O}\\
GJ	15A	&	Johnson	&	V	&	8.09	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	15A	&	Johnson	&	V	&	8.07	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	15A	&	Johnson	&	V	&	8.11	&	0.05	&	\citet{1974PASP...86..294U}\\
GJ	15A	&	Johnson	&	V	&	8.13	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	15A	&	Johnson	&	V	&	8.11	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	15A	&	Johnson	&	V	&	8.07	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	15A	&	Johnson	&	V	&	8.09	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	15A	&	Cousins	&	Rc	&	7.14	&	0.05	&	\citet{1995yCat.5070....0G}\\
GJ	15A	&	Cousins	&	Ic	&	6.02	&	0.05	&	\citet{1995yCat.5070....0G}\\
GJ	15A	&	1020	&	204	&	5.4	&	0.05	&	\citet{1968ApJS...16...49E}\\
GJ	15A	&	Johnson	&	H	&	4.25	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	15A	&	Johnson	&	H	&	4.25	&	0.05	&	\citet{1977AJ.....82..729P}\\
GJ	15A	&	2Mass	&	Ks	&	4.02	&	0.05	&	\citet{2003tmc..book.....C}\\
GJ	15A	&	Johnson	&	K	&	4.01	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	15A	&	Johnson	&	K	&	4.03	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	15A	&	Johnson	&	K	&	4.02	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	15A	&	Johnson	&	K	&	4.04	&	0.05	&	\citet{1977AJ.....82..729P}\\
											
GJ	33	&	Geneva	&	U	&	7.63	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	33	&	Stromgren	&	u	&	8.39	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	33	&	Stromgren	&	u	&	8.38	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	33	&	Stromgren	&	u	&	8.4	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	33	&	Stromgren	&	u	&	8.4	&	0.08	&	\citet{1994A_AS..104..429O}\\
GJ	33	&	Stromgren	&	u	&	8.37	&	0.08	&	\citet{1990A_AS...82..531F}\\
GJ	33	&	Stromgren	&	u	&	8.37	&	0.08	&	\citet{1974AJ.....79.1424O}\\
GJ	33	&	Johnson	&	U	&	7.24	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	33	&	Johnson	&	U	&	7.22	&	0.05	&	\citet{1957ApJ...126..113J}\\
GJ	33	&	Johnson	&	U	&	7.23	&	0.05	&	\citet{1962MNSSA..21...20C}\\
GJ	33	&	Johnson	&	U	&	7.22	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	33	&	Johnson	&	U	&	7.21	&	0.05	&	\citet{1984SAAOC...8...59C}\\
GJ	33	&	Johnson	&	U	&	7.23	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	33	&	Johnson	&	U	&	7.22	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	33	&	Geneva	&	B1	&	7.14	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	33	&	Stromgren	&	v	&	7.2	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	33	&	Stromgren	&	v	&	7.19	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	33	&	Stromgren	&	v	&	7.2	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	33	&	Stromgren	&	v	&	7.2	&	0.08	&	\citet{1994A_AS..104..429O}\\
GJ	33	&	Stromgren	&	v	&	7.2	&	0.08	&	\citet{1990A_AS...82..531F}\\
GJ	33	&	Stromgren	&	v	&	7.17	&	0.08	&	\citet{1974AJ.....79.1424O}\\
GJ	33	&	Geneva	&	B	&	5.89	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	33	&	Geneva	&	B2	&	7.07	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	33	&	Johnson	&	B	&	6.64	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	33	&	Johnson	&	B	&	6.64	&	0.05	&	\citet{1957ApJ...126..113J}\\
GJ	33	&	Johnson	&	B	&	6.61	&	0.05	&	\citet{1962MNSSA..21...20C}\\
GJ	33	&	Johnson	&	B	&	6.64	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	33	&	Johnson	&	B	&	6.63	&	0.05	&	\citet{1984SAAOC...8...59C}\\
GJ	33	&	Johnson	&	B	&	6.63	&	0.05	&	\citet{1961ApJS....6..253I}\\
GJ	33	&	Johnson	&	B	&	6.63	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	33	&	Johnson	&	B	&	6.64	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	33	&	Stromgren	&	b	&	6.26	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	33	&	Stromgren	&	b	&	6.26	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	33	&	Stromgren	&	b	&	6.26	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	33	&	Stromgren	&	b	&	6.26	&	0.08	&	\citet{1994A_AS..104..429O}\\
GJ	33	&	Stromgren	&	b	&	6.27	&	0.08	&	\citet{1990A_AS...82..531F}\\
GJ	33	&	Stromgren	&	b	&	6.27	&	0.08	&	\citet{1974AJ.....79.1424O}\\
GJ	33	&	Geneva	&	V1	&	6.52	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	33	&	Stromgren	&	y	&	5.75	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	33	&	Stromgren	&	y	&	5.75	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	33	&	Stromgren	&	y	&	5.75	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	33	&	Stromgren	&	y	&	5.75	&	0.08	&	\citet{1994A_AS..104..429O}\\
GJ	33	&	Stromgren	&	y	&	5.75	&	0.08	&	\citet{1990A_AS...82..531F}\\
GJ	33	&	Stromgren	&	y	&	5.75	&	0.08	&	\citet{1974AJ.....79.1424O}\\
GJ	33	&	Geneva	&	V	&	5.75	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	33	&	Johnson	&	V	&	5.74	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	33	&	Johnson	&	V	&	5.76	&	0.05	&	\citet{1957ApJ...126..113J}\\
GJ	33	&	Johnson	&	V	&	5.72	&	0.05	&	\citet{1962MNSSA..21...20C}\\
GJ	33	&	Johnson	&	V	&	5.76	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	33	&	Johnson	&	V	&	5.73	&	0.05	&	\citet{1984SAAOC...8...59C}\\
GJ	33	&	Johnson	&	V	&	5.72	&	0.05	&	\citet{1961ApJS....6..253I}\\
GJ	33	&	Johnson	&	V	&	5.74	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	33	&	Johnson	&	V	&	5.76	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	33	&	Geneva	&	G	&	6.71	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	33	&	Johnson	&	R	&	4.99	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	33	&	Johnson	&	I	&	4.52	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	33	&	1250	&	250	&	4.24	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	33	&	2Mass	&	J	&	4.37	&	0.31	&	\citet{2003tmc..book.....C}\\
GJ	33	&	Johnson	&	J	&	4.24	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	33	&	1650	&	330	&	3.72	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	33	&	2Mass	&	H	&	3.72	&	0.23	&	\citet{2003tmc..book.....C}\\
GJ	33	&	Johnson	&	H	&	3.72	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	33	&	2Mass	&	Ks	&	3.68	&	0.27	&	\citet{2003tmc..book.....C}\\
GJ	33	&	2200	&	440	&	3.61	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	33	&	Johnson	&	K	&	3.61	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	33	&	3500	&	700	&	3.48	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	33	&	Johnson	&	L	&	3.48	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	53A	&	Stromgren	&	u	&	7.04	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	53A	&	Stromgren	&	u	&	7.05	&	0.08	&	\citet{1988A_AS...73..225S}\\
GJ	53A	&	Stromgren	&	u	&	7.05	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	53A	&	Stromgren	&	u	&	7.05	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	53A	&	Stromgren	&	u	&	7.06	&	0.08	&	\citet{1970AJ.....75..978C}\\
GJ	53A	&	Stromgren	&	u	&	7.07	&	0.08	&	\citet{1970ApJS...22..117B}\\
GJ	53A	&	Stromgren	&	u	&	7.09	&	0.08	&	\citet{1993PASP..105...36S}\\
GJ	53A	&	Johnson	&	U	&	5.9	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	53A	&	Johnson	&	U	&	5.93	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	53A	&	Johnson	&	U	&	5.96	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	53A	&	Johnson	&	U	&	5.96	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	53A	&	Johnson	&	U	&	5.96	&	0.05	&	\citet{1979AJ.....84..867C}\\
GJ	53A	&	Johnson	&	U	&	5.96	&	0.05	&	\citet{1979ApJ...233..211C}\\
GJ	53A	&	Johnson	&	U	&	5.97	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	53A	&	Johnson	&	U	&	5.98	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	53A	&	Johnson	&	U	&	6.02	&	0.05	&	\citet{1955ApJS....2..195R}\\
GJ	53A	&	Stromgren	&	v	&	6.19	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	53A	&	Stromgren	&	v	&	6.19	&	0.08	&	\citet{1988A_AS...73..225S}\\
GJ	53A	&	Stromgren	&	v	&	6.2	&	0.08	&	\citet{1970ApJS...22..117B}\\
GJ	53A	&	Stromgren	&	v	&	6.2	&	0.08	&	\citet{1970AJ.....75..978C}\\
GJ	53A	&	Stromgren	&	v	&	6.2	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	53A	&	Stromgren	&	v	&	6.2	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	53A	&	Stromgren	&	v	&	6.22	&	0.08	&	\citet{1993PASP..105...36S}\\
GJ	53A	&	Johnson	&	B	&	5.81	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	53A	&	Johnson	&	B	&	5.84	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	53A	&	Johnson	&	B	&	5.85	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	53A	&	Johnson	&	B	&	5.85	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	53A	&	Johnson	&	B	&	5.86	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	53A	&	Johnson	&	B	&	5.86	&	0.05	&	\citet{1979AJ.....84..867C}\\
GJ	53A	&	Johnson	&	B	&	5.86	&	0.05	&	\citet{1979ApJ...233..211C}\\
GJ	53A	&	Johnson	&	B	&	5.87	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	53A	&	Johnson	&	B	&	5.87	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	53A	&	Johnson	&	B	&	5.88	&	0.05	&	\citet{1963ArA.....3..273O}\\
GJ	53A	&	Johnson	&	B	&	5.91	&	0.05	&	\citet{1955ApJS....2..195R}\\
GJ	53A	&	Stromgren	&	b	&	5.55	&	0.08	&	\citet{1970AJ.....75..978C}\\
GJ	53A	&	Stromgren	&	b	&	5.55	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	53A	&	Stromgren	&	b	&	5.56	&	0.08	&	\citet{1970ApJS...22..117B}\\
GJ	53A	&	Stromgren	&	b	&	5.56	&	0.08	&	\citet{1988A_AS...73..225S}\\
GJ	53A	&	Stromgren	&	b	&	5.56	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	53A	&	Stromgren	&	b	&	5.56	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	53A	&	Stromgren	&	b	&	5.56	&	0.08	&	\citet{1993PASP..105...36S}\\
GJ	53A	&	Stromgren	&	y	&	5.12	&	0.08	&	\citet{1970AJ.....75..978C}\\
GJ	53A	&	Stromgren	&	y	&	5.12	&	0.08	&	\citet{1970ApJS...22..117B}\\
GJ	53A	&	Stromgren	&	y	&	5.12	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	53A	&	Stromgren	&	y	&	5.12	&	0.08	&	\citet{1988A_AS...73..225S}\\
GJ	53A	&	Stromgren	&	y	&	5.12	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	53A	&	Stromgren	&	y	&	5.12	&	0.08	&	\citet{1993PASP..105...36S}\\
GJ	53A	&	Stromgren	&	y	&	5.12	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	53A	&	Johnson	&	V	&	5.12	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	53A	&	Johnson	&	V	&	5.15	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	53A	&	Johnson	&	V	&	5.15	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	53A	&	Johnson	&	V	&	5.16	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	53A	&	Johnson	&	V	&	5.16	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	53A	&	Johnson	&	V	&	5.16	&	0.05	&	\citet{1979AJ.....84..867C}\\
GJ	53A	&	Johnson	&	V	&	5.16	&	0.05	&	\citet{1979ApJ...233..211C}\\
GJ	53A	&	Johnson	&	V	&	5.17	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	53A	&	Johnson	&	V	&	5.18	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	53A	&	Johnson	&	V	&	5.2	&	0.05	&	\citet{1955ApJS....2..195R}\\
GJ	53A	&	Johnson	&	V	&	5.21	&	0.05	&	\citet{1963ArA.....3..273O}\\
GJ	53A	&	Johnson	&	R	&	4.55	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	53A	&	Johnson	&	R	&	4.55	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	53A	&	Johnson	&	I	&	4.12	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	53A	&	Johnson	&	I	&	4.14	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	53A	&	1250	&	250	&	3.76	&	0.05	&	\citet{1983AJ.....88..623C}\\
GJ	53A	&	1250	&	250	&	3.79	&	0.05	&	\citet{1979AJ.....84..867C}\\
GJ	53A	&	1250	&	250	&	3.86	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	53A	&	1250	&	250	&	3.86	&	0.05	&	\citet{1975A_AS...22....1V}\\
GJ	53A	&	1280	&	256	&	3.77	&	0.05	&	\citet{1994A_AS..107..365A}\\
GJ	53A	&	1650	&	330	&	3.39	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	53A	&	1650	&	330	&	3.39	&	0.05	&	\citet{1975A_AS...22....1V}\\
GJ	53A	&	1650	&	330	&	3.4	&	0.05	&	\citet{1979AJ.....84..867C}\\
GJ	53A	&	1650	&	330	&	3.4	&	0.05	&	\citet{1983AJ.....88..623C}\\
GJ	53A	&	1650	&	330	&	3.39	&	0.05	&	\citet{1994A_AS..107..365A}\\
GJ	53A	&	2190	&	438	&	3.33	&	0.05	&	\citet{1994A_AS..107..365A}\\
GJ	53A	&	2200	&	440	&	3.3	&	0.05	&	\citet{1984AJ.....89..433M}\\
GJ	53A	&	2200	&	440	&	3.34	&	0.05	&	\citet{1979AJ.....84..867C}\\
GJ	53A	&	2200	&	440	&	3.34	&	0.05	&	\citet{1983AJ.....88..623C}\\
GJ	53A	&	2200	&	440	&	3.36	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	53A	&	2200	&	440	&	3.36	&	0.05	&	\citet{1975A_AS...22....1V}\\
GJ	53A	&	3400	&	680	&	3.4	&	0.05	&	\citet{1984AJ.....89..433M}\\
GJ	53A	&	3500	&	700	&	3.3	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	53A	&	3500	&	700	&	3.3	&	0.05	&	\citet{1975A_AS...22....1V}\\
GJ	75	&	Stromgren	&	u	&	7.99	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	75	&	Stromgren	&	u	&	8.01	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	75	&	Stromgren	&	u	&	8.03	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	75	&	Johnson	&	U	&	6.83	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	75	&	Johnson	&	U	&	6.83	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	75	&	Johnson	&	U	&	6.83	&	0.05	&	\citet{1975MNRAS.172..667J}\\
GJ	75	&	Johnson	&	U	&	6.84	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	75	&	Johnson	&	U	&	6.84	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	75	&	Johnson	&	U	&	6.86	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	75	&	Stromgren	&	v	&	6.88	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	75	&	Stromgren	&	v	&	6.9	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	75	&	Stromgren	&	v	&	6.91	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	75	&	Johnson	&	B	&	6.41	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	75	&	Johnson	&	B	&	6.42	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	75	&	Johnson	&	B	&	6.43	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	75	&	Johnson	&	B	&	6.43	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	75	&	Johnson	&	B	&	6.43	&	0.05	&	\citet{1975MNRAS.172..667J}\\
GJ	75	&	Johnson	&	B	&	6.44	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	75	&	Johnson	&	B	&	6.44	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	75	&	Stromgren	&	b	&	6.1	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	75	&	Stromgren	&	b	&	6.1	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	75	&	Stromgren	&	b	&	6.11	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	75	&	Stromgren	&	y	&	5.63	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	75	&	Stromgren	&	y	&	5.63	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	75	&	Stromgren	&	y	&	5.63	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	75	&	Johnson	&	V	&	5.59	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	75	&	Johnson	&	V	&	5.63	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	75	&	Johnson	&	V	&	5.63	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	75	&	Johnson	&	V	&	5.63	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	75	&	Johnson	&	V	&	5.63	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	75	&	Johnson	&	V	&	5.64	&	0.05	&	\citet{1975MNRAS.172..667J}\\
GJ	75	&	Johnson	&	V	&	5.64	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	75	&	Johnson	&	R	&	4.99	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	75	&	Johnson	&	I	&	4.6	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	75	&	1250	&	250	&	4.31	&	0.05	&	\citet{1989A_A...215..305A}\\
GJ	75	&	1650	&	330	&	3.88	&	0.05	&	\citet{1989A_A...215..305A}\\
GJ	75	&	2200	&	440	&	3.84	&	0.05	&	\citet{1989A_A...215..305A}\\
GJ	75	&	3400	&	680	&	3.7	&	0.05	&	\citet{1989A_A...215..305A}\\
GJ	105A	&	Johnson	&	U	&	7.58	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	105A	&	Johnson	&	U	&	7.59	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	105A	&	Johnson	&	U	&	7.6	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	105A	&	Johnson	&	U	&	7.58	&	0.05	&	\citet{1955ApJS....2..195R}\\
GJ	105A	&	Johnson	&	U	&	7.58	&	0.05	&	\citet{1954ApJ...120..196J}\\
GJ	105A	&	Johnson	&	U	&	7.65	&	0.05	&	\citet{1963MNSSA..22...12C}\\
GJ	105A	&	Johnson	&	U	&	7.59	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	105A	&	Johnson	&	U	&	7.6	&	0.05	&	\citet{1984SAAOC...8...59C}\\
GJ	105A	&	Johnson	&	U	&	7.58	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	105A	&	Johnson	&	U	&	7.61	&	0.05	&	\citet{1971A_A....12..442M}\\
GJ	105A	&	Johnson	&	B	&	6.81	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	105A	&	Johnson	&	B	&	6.79	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	105A	&	Johnson	&	B	&	6.81	&	0.05	&	\citet{1955ApJS....2..195R}\\
GJ	105A	&	Johnson	&	B	&	6.79	&	0.05	&	\citet{1954ApJ...120..196J}\\
GJ	105A	&	Johnson	&	B	&	6.84	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	105A	&	Johnson	&	B	&	6.77	&	0.05	&	\citet{1963MNSSA..22...12C}\\
GJ	105A	&	Johnson	&	B	&	6.79	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	105A	&	Johnson	&	B	&	6.79	&	0.05	&	\citet{1984SAAOC...8...59C}\\
GJ	105A	&	Johnson	&	B	&	6.79	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	105A	&	Johnson	&	B	&	6.78	&	0.05	&	\citet{1971A_A....12..442M}\\
GJ	105A	&	Johnson	&	B	&	6.79	&	0.05	&	\citet{1970BOTT....5..269M}\\
GJ	105A	&	Johnson	&	B	&	6.81	&	0.05	&	\citet{1969BOTT....5...57M}\\
GJ	105A	&	Johnson	&	V	&	5.82	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	105A	&	Johnson	&	V	&	5.82	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	105A	&	Johnson	&	V	&	5.82	&	0.05	&	\citet{1955ApJS....2..195R}\\
GJ	105A	&	Johnson	&	V	&	5.82	&	0.05	&	\citet{1954ApJ...120..196J}\\
GJ	105A	&	Johnson	&	V	&	5.86	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	105A	&	Johnson	&	V	&	5.79	&	0.05	&	\citet{1963MNSSA..22...12C}\\
GJ	105A	&	Johnson	&	V	&	5.84	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	105A	&	Johnson	&	V	&	5.8	&	0.05	&	\citet{1984SAAOC...8...59C}\\
GJ	105A	&	Johnson	&	V	&	5.82	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	105A	&	Johnson	&	V	&	5.83	&	0.05	&	\citet{1971A_A....12..442M}\\
GJ	105A	&	Johnson	&	V	&	5.82	&	0.05	&	\citet{1970BOTT....5..269M}\\
GJ	105A	&	Johnson	&	V	&	5.83	&	0.05	&	\citet{1969BOTT....5...57M}\\
GJ	105A	&	Johnson	&	R	&	4.99	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	105A	&	Johnson	&	R	&	5.04	&	0.05	&	\citet{1971A_A....12..442M}\\
GJ	105A	&	Johnson	&	R	&	4.98	&	0.05	&	\citet{1970BOTT....5..269M}\\
GJ	105A	&	Johnson	&	R	&	5.01	&	0.05	&	\citet{1969BOTT....5...57M}\\
GJ	105A	&	Johnson	&	R	&	4.99	&	0.05	&	\citet{1967BOTT....4..106M}\\
GJ	105A	&	Johnson	&	I	&	4.46	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	105A	&	Johnson	&	I	&	4.45	&	0.05	&	\citet{1970BOTT....5..269M}\\
GJ	105A	&	Johnson	&	I	&	4.49	&	0.05	&	\citet{1969BOTT....5...57M}\\
GJ	105A	&	Johnson	&	I	&	4.46	&	0.05	&	\citet{1967BOTT....4..106M}\\
GJ	105A	&	1250	&	250	&	4.07	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	105A	&	1250	&	250	&	4.15	&	0.05	&	\citet{1996ApJ...458L..41R}\\
GJ	105A	&	2Mass	&	J	&	4.15	&	0.26	&	\citet{2003tmc..book.....C}\\
GJ	105A	&	Johnson	&	J	&	4.07	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	105A	&	1280	&	256	&	3.99	&	0.05	&	\citet{1994A_AS..107..365A}\\
GJ	105A	&	1650	&	330	&	3.52	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	105A	&	1650	&	330	&	3.48	&	0.05	&	\citet{1994A_AS..107..365A}\\
GJ	105A	&	1650	&	330	&	3.61	&	0.05	&	\citet{1996ApJ...458L..41R}\\
GJ	105A	&	2Mass	&	H	&	3.66	&	0.24	&	\citet{2003tmc..book.....C}\\
GJ	105A	&	Johnson	&	H	&	3.52	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	105A	&	2160	&	432	&	3.52	&	0.05	&	\citet{1996ApJ...458L..41R}\\
GJ	105A	&	2Mass	&	Ks	&	3.48	&	0.21	&	\citet{2003tmc..book.....C}\\
GJ	105A	&	2190	&	438	&	3.4	&	0.05	&	\citet{1994A_AS..107..365A}\\
GJ	105A	&	2200	&	440	&	3.45	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	105A	&	Johnson	&	K	&	3.45	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	105A	&	3400	&	680	&	3.43	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	105A	&	Johnson	&	L	&	3.43	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
											
GJ	144	&	Geneva	&	U	&	5.63	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	144	&	Stromgren	&	u	&	6.35	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	144	&	Stromgren	&	u	&	6.37	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	144	&	Stromgren	&	u	&	6.37	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	144	&	Stromgren	&	u	&	6.38	&	0.08	&	\citet{1984A_AS...57..443O}\\
GJ	144	&	Johnson	&	U	&	14.55	&	0.1	&	\citet{1986EgUBV........0M}\\
GJ	144	&	Johnson	&	U	&	14.56	&	0.1	&	\citet{1972PASP...84..581F}\\
GJ	144	&	Johnson	&	U	&	5.18	&	0.05	&	\citet{1966PDAUC...1....1G}\\
GJ	144	&	Johnson	&	U	&	5.19	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	144	&	Johnson	&	U	&	5.19	&	0.05	&	\citet{1954ApJ...120..196J}\\
GJ	144	&	Johnson	&	U	&	5.19	&	0.05	&	\citet{1963MNRAS.125..199T}\\
GJ	144	&	Johnson	&	U	&	5.19	&	0.05	&	\citet{1964BOTT....3..305J}\\
GJ	144	&	Johnson	&	U	&	5.19	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	144	&	Johnson	&	U	&	5.19	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	144	&	Johnson	&	U	&	5.19	&	0.05	&	\citet{1984SAAOC...8...59C}\\
GJ	144	&	Johnson	&	U	&	5.2	&	0.05	&	\citet{1978AJ.....83..606M}\\
GJ	144	&	Johnson	&	U	&	5.2	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	144	&	Johnson	&	U	&	5.21	&	0.05	&	\citet{1971A_A....12..442M}\\
GJ	144	&	Johnson	&	U	&	5.22	&	0.05	&	\citet{1958MtSOM...2....1H}\\
GJ	144	&	Johnson	&	U	&	5.22	&	0.05	&	\citet{1962RGOB...64..103C}\\
GJ	144	&	Geneva	&	B1	&	5.12	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	144	&	Stromgren	&	v	&	5.16	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	144	&	Stromgren	&	v	&	5.17	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	144	&	Stromgren	&	v	&	5.17	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	144	&	Stromgren	&	v	&	5.18	&	0.08	&	\citet{1984A_AS...57..443O}\\
GJ	144	&	Geneva	&	B	&	3.87	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	144	&	Johnson	&	B	&	4.58	&	0.05	&	\citet{1969BOTT....5...57M}\\
GJ	144	&	Johnson	&	B	&	4.58	&	0.05	&	\citet{1952ApJ...116..251S}\\
GJ	144	&	Johnson	&	B	&	4.59	&	0.05	&	\citet{1971A_A....12..442M}\\
GJ	144	&	Johnson	&	B	&	4.6	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	144	&	Johnson	&	B	&	4.6	&	0.05	&	\citet{1959ApJ...129..647P}\\
GJ	144	&	Johnson	&	B	&	4.6	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	144	&	Johnson	&	B	&	4.6	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	144	&	Johnson	&	B	&	4.61	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	144	&	Johnson	&	B	&	4.61	&	0.05	&	\citet{1970BOTT....5..269M}\\
GJ	144	&	Johnson	&	B	&	4.61	&	0.05	&	\citet{1962RGOB...64..103C}\\
GJ	144	&	Johnson	&	B	&	4.61	&	0.05	&	\citet{1963MNRAS.125..199T}\\
GJ	144	&	Johnson	&	B	&	4.62	&	0.05	&	\citet{1966PDAUC...1....1G}\\
GJ	144	&	Johnson	&	B	&	4.62	&	0.05	&	\citet{1954ApJ...120..196J}\\
GJ	144	&	Johnson	&	B	&	4.62	&	0.05	&	\citet{1964BOTT....3..305J}\\
GJ	144	&	Johnson	&	B	&	4.62	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	144	&	Johnson	&	B	&	4.62	&	0.05	&	\citet{1978AJ.....83..606M}\\
GJ	144	&	Johnson	&	B	&	4.62	&	0.05	&	\citet{1984SAAOC...8...59C}\\
GJ	144	&	Johnson	&	B	&	4.63	&	0.05	&	\citet{1958MtSOM...2....1H}\\
GJ	144	&	Geneva	&	B2	&	5.07	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	144	&	Stromgren	&	b	&	4.23	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	144	&	Stromgren	&	b	&	4.23	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	144	&	Stromgren	&	b	&	4.24	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	144	&	Stromgren	&	b	&	4.24	&	0.08	&	\citet{1984A_AS...57..443O}\\
GJ	144	&	Geneva	&	V1	&	4.51	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	144	&	Stromgren	&	y	&	3.73	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	144	&	Stromgren	&	y	&	3.73	&	0.08	&	\citet{1984A_AS...57..443O}\\
GJ	144	&	Stromgren	&	y	&	3.73	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	144	&	Stromgren	&	y	&	3.73	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	144	&	Geneva	&	V	&	3.73	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	144	&	Johnson	&	V	&	3.7	&	0.05	&	\citet{1969BOTT....5...57M}\\
GJ	144	&	Johnson	&	V	&	3.71	&	0.05	&	\citet{1952ApJ...116..251S}\\
GJ	144	&	Johnson	&	V	&	3.71	&	0.05	&	\citet{1962RGOB...64..103C}\\
GJ	144	&	Johnson	&	V	&	3.72	&	0.05	&	\citet{1971A_A....12..442M}\\
GJ	144	&	Johnson	&	V	&	3.72	&	0.05	&	\citet{1959ApJ...129..647P}\\
GJ	144	&	Johnson	&	V	&	3.72	&	0.05	&	\citet{1962RGOB...64..103C}\\
GJ	144	&	Johnson	&	V	&	3.72	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	144	&	Johnson	&	V	&	3.72	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	144	&	Johnson	&	V	&	3.73	&	0.05	&	\citet{1966PDAUC...1....1G}\\
GJ	144	&	Johnson	&	V	&	3.73	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	144	&	Johnson	&	V	&	3.73	&	0.05	&	\citet{1970BOTT....5..269M}\\
GJ	144	&	Johnson	&	V	&	3.73	&	0.05	&	\citet{1954ApJ...120..196J}\\
GJ	144	&	Johnson	&	V	&	3.73	&	0.05	&	\citet{1963MNRAS.125..199T}\\
GJ	144	&	Johnson	&	V	&	3.73	&	0.05	&	\citet{1964BOTT....3..305J}\\
GJ	144	&	Johnson	&	V	&	3.73	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	144	&	Johnson	&	V	&	3.74	&	0.05	&	\citet{1984SAAOC...8...59C}\\
GJ	144	&	Johnson	&	V	&	3.74	&	0.05	&	\citet{1978AJ.....83..606M}\\
GJ	144	&	Johnson	&	V	&	3.75	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	144	&	Johnson	&	V	&	3.75	&	0.05	&	\citet{1958MtSOM...2....1H}\\
GJ	144	&	Geneva	&	G	&	4.71	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	144	&	Johnson	&	R	&	2.97	&	0.05	&	\citet{1969BOTT....5...57M}\\
GJ	144	&	Johnson	&	R	&	3.01	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	144	&	Johnson	&	R	&	3.01	&	0.05	&	\citet{1967BOTT....4..106M}\\
GJ	144	&	Johnson	&	R	&	3.01	&	0.05	&	\citet{1970BOTT....5..269M}\\
GJ	144	&	Johnson	&	R	&	3.02	&	0.05	&	\citet{1971A_A....12..442M}\\
GJ	144	&	Johnson	&	I	&	2.51	&	0.05	&	\citet{1969BOTT....5...57M}\\
GJ	144	&	Johnson	&	I	&	2.54	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	144	&	Johnson	&	I	&	2.54	&	0.05	&	\citet{1967BOTT....4..106M}\\
GJ	144	&	Johnson	&	I	&	2.54	&	0.05	&	\citet{1970BOTT....5..269M}\\
GJ	144	&	1200	&	240	&	2.2	&	0.05	&	\citet{1974MNSSA..33...53G}\\
GJ	144	&	1250	&	250	&	2.17	&	0.05	&	\citet{1989A_A...215..305A}\\
GJ	144	&	1250	&	250	&	2.2	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	144	&	1250	&	250	&	2.24	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	144	&	1250	&	250	&	2.24	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	144	&	1250	&	250	&	2.26	&	0.05	&	\citet{1981A_AS...45....5E}\\
GJ	144	&	1250	&	250	&	2.26	&	0.05	&	\citet{1984RMxAA...9...65T}\\
GJ	144	&	1250	&	250	&	2.27	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	144	&	1250	&	250	&	2.29	&	0.05	&	\citet{1987ApJ...320..850V}\\
GJ	144	&	1250	&	250	&	5.34	&	0.05	&	\citet{1991AJ....101..662B}\\
GJ	144	&	1250	&	250	&	5.39	&	0.05	&	\citet{1991ApJ...368..264A}\\
GJ	144	&	1250	&	250	&	2.23	&	0.05	&	\citet{1990MNRAS.242....1C}\\
GJ	144	&	1250	&	250	&	5.33	&	0.05	&	\citet{1976ApJ...208..399M}\\
GJ	144	&	1600	&	320	&	1.75	&	0.05	&	\citet{1974MNSSA..33...53G}\\
GJ	144	&	1600	&	320	&	4.73	&	0.05	&	\citet{1972PASP...84..581F}\\
GJ	144	&	1650	&	330	&	1.69	&	0.05	&	\citet{1989A_A...215..305A}\\
GJ	144	&	1650	&	330	&	1.75	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	144	&	1650	&	330	&	1.77	&	0.05	&	\citet{1987ApJ...320..850V}\\
GJ	144	&	1650	&	330	&	1.79	&	0.05	&	\citet{1981A_AS...45....5E}\\
GJ	144	&	1650	&	330	&	1.79	&	0.05	&	\citet{1984RMxAA...9...65T}\\
GJ	144	&	1650	&	330	&	4.71	&	0.05	&	\citet{1991AJ....101..662B}\\
GJ	144	&	1650	&	330	&	4.73	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	144	&	1650	&	330	&	4.74	&	0.05	&	\citet{1991ApJ...368..264A}\\
GJ	144	&	1650	&	330	&	1.72	&	0.05	&	\citet{1990MNRAS.242....1C}\\
GJ	144	&	1650	&	330	&	4.73	&	0.05	&	\citet{1976ApJ...208..399M}\\
GJ	144	&	2200	&	440	&	1.65	&	0.05	&	\citet{1974MNSSA..33...53G}\\
GJ	144	&	2200	&	440	&	1.65	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	144	&	2200	&	440	&	1.66	&	0.05	&	\citet{1989A_A...215..305A}\\
GJ	144	&	2200	&	440	&	1.68	&	0.05	&	\citet{1987ApJ...320..850V}\\
GJ	144	&	2200	&	440	&	1.69	&	0.05	&	\citet{1981A_AS...45....5E}\\
GJ	144	&	2200	&	440	&	1.69	&	0.05	&	\citet{1984RMxAA...9...65T}\\
GJ	144	&	2200	&	440	&	1.7	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	144	&	2200	&	440	&	1.7	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	144	&	2200	&	440	&	1.73	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	144	&	2200	&	440	&	4.36	&	0.05	&	\citet{1991AJ....101..662B}\\
GJ	144	&	2200	&	440	&	4.38	&	0.05	&	\citet{1991ApJ...368..264A}\\
GJ	144	&	2200	&	440	&	4.4	&	0.05	&	\citet{1972PASP...84..581F}\\
GJ	144	&	2200	&	440	&	4.4	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	144	&	2200	&	440	&	1.66	&	0.05	&	\citet{1990MNRAS.242....1C}\\
GJ	144	&	2200	&	440	&	4.37	&	0.05	&	\citet{1976ApJ...208..399M}\\
GJ	144	&	2300	&	460	&	4.6	&	0.05	&	\citet{1972PASP...84..581F}\\
GJ	144	&	3400	&	680	&	4.1	&	0.05	&	\citet{1972PASP...84..581F}\\
GJ	144	&	3400	&	680	&	1.5	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	144	&	3400	&	680	&	1.53	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	144	&	3400	&	680	&	1.59	&	0.05	&	\citet{1989A_A...215..305A}\\
GJ	144	&	3400	&	680	&	1.6	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	144	&	3400	&	680	&	1.61	&	0.05	&	\citet{1974MNSSA..33...53G}\\
GJ	144	&	3400	&	680	&	1.68	&	0.05	&	\citet{1987ApJ...320..850V}\\
GJ	144	&	3400	&	680	&	4.15	&	0.05	&	\citet{1991ApJ...368..264A}\\
GJ	144	&	3400	&	680	&	1.62	&	0.05	&	\citet{1990MNRAS.242....1C}\\
GJ	144	&	3500	&	700	&	4.2	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	144	&	3500	&	700	&	4.17	&	0.05	&	\citet{1972PASP...84..581F}\\
GJ	144	&	3500	&	700	&	4.04	&	0.05	&	\citet{1976ApJ...208..399M}\\
GJ	144	&	Johnson	&	M	&	4.8	&	0.05	&	\citet{1972PASP...84..581F}\\
GJ	166A	&	Geneva	&	U	&	6.11	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	166A	&	Stromgren	&	u	&	6.83	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	166A	&	Stromgren	&	u	&	6.81	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	166A	&	Stromgren	&	u	&	6.83	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	166A	&	Stromgren	&	u	&	6.84	&	0.08	&	\citet{1988A_AS...73..225S}\\
GJ	166A	&	Stromgren	&	u	&	6.83	&	0.08	&	\citet{1990A_AS...82..531F}\\
GJ	166A	&	Stromgren	&	u	&	6.83	&	0.08	&	\citet{1977A_AS...29..313O}\\
GJ	166A	&	Johnson	&	U	&	5.68	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	166A	&	Johnson	&	U	&	5.69	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	166A	&	Geneva	&	B1	&	5.66	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	166A	&	Stromgren	&	v	&	5.71	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	166A	&	Stromgren	&	v	&	5.71	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	166A	&	Stromgren	&	v	&	5.71	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	166A	&	Stromgren	&	v	&	5.71	&	0.08	&	\citet{1988A_AS...73..225S}\\
GJ	166A	&	Stromgren	&	v	&	5.72	&	0.08	&	\citet{1990A_AS...82..531F}\\
GJ	166A	&	Stromgren	&	v	&	5.71	&	0.08	&	\citet{1977A_AS...29..313O}\\
GJ	166A	&	Geneva	&	B	&	4.47	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	166A	&	Geneva	&	B2	&	5.7	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	166A	&	Johnson	&	B	&	5.23	&	0.05	&	\citet{1962RGOB...64..103C}\\
GJ	166A	&	Johnson	&	B	&	5.22	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	166A	&	Johnson	&	B	&	5.25	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	166A	&	Stromgren	&	b	&	4.89	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	166A	&	Stromgren	&	b	&	4.89	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	166A	&	Stromgren	&	b	&	4.9	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	166A	&	Stromgren	&	b	&	4.9	&	0.08	&	\citet{1988A_AS...73..225S}\\
GJ	166A	&	Stromgren	&	b	&	4.9	&	0.08	&	\citet{1990A_AS...82..531F}\\
GJ	166A	&	Stromgren	&	b	&	4.9	&	0.08	&	\citet{1977A_AS...29..313O}\\
GJ	166A	&	Geneva	&	V1	&	5.19	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	166A	&	Stromgren	&	y	&	4.41	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	166A	&	Stromgren	&	y	&	4.41	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	166A	&	Stromgren	&	y	&	4.41	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	166A	&	Stromgren	&	y	&	4.41	&	0.08	&	\citet{1988A_AS...73..225S}\\
GJ	166A	&	Stromgren	&	y	&	4.41	&	0.08	&	\citet{1990A_AS...82..531F}\\
GJ	166A	&	Stromgren	&	y	&	4.41	&	0.08	&	\citet{1977A_AS...29..313O}\\
GJ	166A	&	Geneva	&	V	&	4.43	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	166A	&	Johnson	&	V	&	4.41	&	0.05	&	\citet{1962RGOB...64..103C}\\
GJ	166A	&	Johnson	&	V	&	4.41	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	166A	&	Johnson	&	V	&	4.43	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	166A	&	Geneva	&	G	&	5.4	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	166A	&	Johnson	&	R	&	3.74	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	166A	&	Johnson	&	I	&	3.29	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	166A	&	1240	&	248	&	2.9	&	0.05	&	\citet{1988A_AS...74..127S}\\
GJ	166A	&	1250	&	250	&	2.95	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	166A	&	1250	&	250	&	2.95	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	166A	&	1250	&	250	&	2.99	&	0.05	&	\citet{1989A_A...215..305A}\\
GJ	166A	&	1250	&	250	&	2.9	&	0.05	&	\citet{1990A_A...232..396B}\\
GJ	166A	&	Johnson	&	J	&	2.95	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	166A	&	Johnson	&	J	&	2.95	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	166A	&	1280	&	256	&	2.85	&	0.05	&	\citet{1994A_AS..107..365A}\\
GJ	166A	&	1650	&	330	&	2.48	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	166A	&	1650	&	330	&	2.48	&	0.05	&	\citet{1989A_A...215..305A}\\
GJ	166A	&	1650	&	330	&	2.42	&	0.05	&	\citet{1994A_AS..107..365A}\\
GJ	166A	&	Johnson	&	H	&	2.48	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	166A	&	2190	&	438	&	2.35	&	0.05	&	\citet{1994A_AS..107..365A}\\
GJ	166A	&	2200	&	440	&	2.4	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	166A	&	2200	&	440	&	2.41	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	166A	&	2200	&	440	&	2.46	&	0.05	&	\citet{1989A_A...215..305A}\\
GJ	166A	&	2200	&	440	&	2.41	&	0.05	&	\citet{1988A_AS...74..127S}\\
GJ	166A	&	2210	&	442	&	2.41	&	0.05	&	\citet{1990A_A...232..396B}\\
GJ	166A	&	Johnson	&	K	&	2.41	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	166A	&	Johnson	&	K	&	2.4	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	166A	&	3400	&	680	&	2.28	&	0.05	&	\citet{1989A_A...215..305A}\\
GJ	166A	&	3500	&	700	&	2.37	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	166A	&	Johnson	&	L	&	2.37	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	205	&	Stromgren	&	u	&	11.9	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	205	&	Stromgren	&	u	&	11.9	&	0.08	&	\citet{1994A_AS..104..429O}\\
GJ	205	&	Stromgren	&	u	&	11.9	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	205	&	Stromgren	&	u	&	11.92	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	205	&	Stromgren	&	u	&	12.25	&	0.08	&	\citet{1966AJ.....71..615W}\\
GJ	205	&	Johnson	&	U	&	10.64	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	205	&	Johnson	&	U	&	10.62	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	205	&	Johnson	&	U	&	10.61	&	0.05	&	\citet{1966ZA.....64..116P}\\
GJ	205	&	Johnson	&	U	&	10.65	&	0.05	&	\citet{1968ArA.....4..433L}\\
GJ	205	&	Johnson	&	U	&	10.71	&	0.05	&	\citet{1972AJ.....77..733B}\\
GJ	205	&	Johnson	&	U	&	10.63	&	0.05	&	\citet{1974PASP...86..294U}\\
GJ	205	&	Johnson	&	U	&	10.67	&	0.05	&	\citet{1983AJ.....88..439L}\\
GJ	205	&	Johnson	&	U	&	10.65	&	0.05	&	\citet{1954ApJ...120..196J}\\
GJ	205	&	Johnson	&	U	&	10.53	&	0.05	&	\citet{1962RGOB...64..103C}\\
GJ	205	&	Johnson	&	U	&	10.72	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	205	&	Johnson	&	U	&	10.61	&	0.05	&	\citet{1984SAAOC...8...59C}\\
GJ	205	&	Johnson	&	U	&	10.66	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	205	&	Johnson	&	U	&	10.65	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	205	&	Stromgren	&	v	&	10.29	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	205	&	Stromgren	&	v	&	10.28	&	0.08	&	\citet{1994A_AS..104..429O}\\
GJ	205	&	Stromgren	&	v	&	10.29	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	205	&	Stromgren	&	v	&	10.32	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	205	&	Stromgren	&	v	&	10.44	&	0.08	&	\citet{1966AJ.....71..615W}\\
GJ	205	&	Johnson	&	B	&	9.44	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	205	&	Johnson	&	B	&	9.49	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	205	&	Johnson	&	B	&	9.44	&	0.05	&	\citet{1966ZA.....64..116P}\\
GJ	205	&	Johnson	&	B	&	9.44	&	0.05	&	\citet{1968ArA.....4..433L}\\
GJ	205	&	Johnson	&	B	&	9.44	&	0.05	&	\citet{1972AJ.....77..733B}\\
GJ	205	&	Johnson	&	B	&	9.44	&	0.05	&	\citet{1974PASP...86..294U}\\
GJ	205	&	Johnson	&	B	&	9.43	&	0.05	&	\citet{1983AJ.....88..439L}\\
GJ	205	&	Johnson	&	B	&	9.44	&	0.05	&	\citet{1952ApJ...116..251S}\\
GJ	205	&	Johnson	&	B	&	9.44	&	0.05	&	\citet{1954ApJ...120..196J}\\
GJ	205	&	Johnson	&	B	&	9.42	&	0.05	&	\citet{1962RGOB...64..103C}\\
GJ	205	&	Johnson	&	B	&	9.45	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	205	&	Johnson	&	B	&	9.49	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	205	&	Johnson	&	B	&	9.47	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	205	&	Johnson	&	B	&	9.44	&	0.05	&	\citet{1984SAAOC...8...59C}\\
GJ	205	&	Johnson	&	B	&	9.45	&	0.05	&	\citet{1958AJ.....63..118A}\\
GJ	205	&	Johnson	&	B	&	9.42	&	0.05	&	\citet{1963MNSSA..22..157S}\\
GJ	205	&	Johnson	&	B	&	9.45	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	205	&	Johnson	&	B	&	9.44	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	205	&	Stromgren	&	b	&	8.84	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	205	&	Stromgren	&	b	&	8.84	&	0.08	&	\citet{1994A_AS..104..429O}\\
GJ	205	&	Stromgren	&	b	&	8.84	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	205	&	Stromgren	&	b	&	8.85	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	205	&	Stromgren	&	b	&	8.93	&	0.08	&	\citet{1966AJ.....71..615W}\\
GJ	205	&	Stromgren	&	y	&	7.92	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	205	&	Stromgren	&	y	&	7.92	&	0.08	&	\citet{1994A_AS..104..429O}\\
GJ	205	&	Stromgren	&	y	&	7.92	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	205	&	Stromgren	&	y	&	7.92	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	205	&	Stromgren	&	y	&	7.92	&	0.08	&	\citet{1966AJ.....71..615W}\\
GJ	205	&	Johnson	&	V	&	7.96	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	205	&	Johnson	&	V	&	7.99	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	205	&	Johnson	&	V	&	7.94	&	0.05	&	\citet{1966ZA.....64..116P}\\
GJ	205	&	Johnson	&	V	&	7.97	&	0.05	&	\citet{1968ArA.....4..433L}\\
GJ	205	&	Johnson	&	V	&	7.97	&	0.05	&	\citet{1972AJ.....77..733B}\\
GJ	205	&	Johnson	&	V	&	7.97	&	0.05	&	\citet{1974PASP...86..294U}\\
GJ	205	&	Johnson	&	V	&	7.96	&	0.05	&	\citet{1983AJ.....88..439L}\\
GJ	205	&	Johnson	&	V	&	7.96	&	0.05	&	\citet{1952ApJ...116..251S}\\
GJ	205	&	Johnson	&	V	&	7.97	&	0.05	&	\citet{1954ApJ...120..196J}\\
GJ	205	&	Johnson	&	V	&	7.94	&	0.05	&	\citet{1962RGOB...64..103C}\\
GJ	205	&	Johnson	&	V	&	7.95	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	205	&	Johnson	&	V	&	7.98	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	205	&	Johnson	&	V	&	8	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	205	&	Johnson	&	V	&	7.95	&	0.05	&	\citet{1984SAAOC...8...59C}\\
GJ	205	&	Johnson	&	V	&	7.98	&	0.05	&	\citet{1958AJ.....63..118A}\\
GJ	205	&	Johnson	&	V	&	7.96	&	0.05	&	\citet{1963MNSSA..22..157S}\\
GJ	205	&	Johnson	&	V	&	7.98	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	205	&	Johnson	&	V	&	7.97	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	205	&	1250	&	250	&	4.72	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	205	&	1250	&	250	&	4.77	&	0.05	&	\citet{1976ApJ...208..399M}\\
GJ	205	&	1250	&	250	&	4.83	&	0.05	&	\citet{1989A_A...215..305A}\\
GJ	205	&	1250	&	250	&	4.75	&	0.05	&	\citet{1994PASP..106..508M}\\
GJ	205	&	1250	&	250	&	4.78	&	0.05	&	\citet{1994PASP..106..508M}\\
GJ	205	&	1250	&	250	&	4.61	&	0.05	&	\citet{1996AJ....112.2238S}\\
GJ	205	&	2Mass	&	J	&	5	&	0.3	&	\citet{2003tmc..book.....C}\\
GJ	205	&	Johnson	&	J	&	4.82	&	0.05	&	\citet{1971BOTT....6..143I}\\
GJ	205	&	Johnson	&	J	&	4.72	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	205	&	Johnson	&	J	&	4.77	&	0.05	&	\citet{1976ApJ...208..399M}\\
GJ	205	&	1650	&	330	&	4.05	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	205	&	1650	&	330	&	4.06	&	0.05	&	\citet{1976ApJ...208..399M}\\
GJ	205	&	1650	&	330	&	4.05	&	0.05	&	\citet{1989A_A...215..305A}\\
GJ	205	&	1650	&	330	&	4.05	&	0.05	&	\citet{1994PASP..106..508M}\\
GJ	205	&	1650	&	330	&	4.08	&	0.05	&	\citet{1994PASP..106..508M}\\
GJ	205	&	1650	&	330	&	3.97	&	0.05	&	\citet{1996AJ....112.2238S}\\
GJ	205	&	2Mass	&	H	&	4.15	&	0.21	&	\citet{2003tmc..book.....C}\\
GJ	205	&	Johnson	&	H	&	4.05	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	205	&	Johnson	&	H	&	4.13	&	0.05	&	\citet{1971BOTT....6..143I}\\
GJ	205	&	Johnson	&	H	&	4.06	&	0.05	&	\citet{1976ApJ...208..399M}\\
GJ	205	&	2100	&	420	&	3.75	&	0.05	&	\citet{1996AJ....112.2238S}\\
GJ	205	&	2Mass	&	Ks	&	4.04	&	0.26	&	\citet{2003tmc..book.....C}\\
GJ	205	&	2200	&	440	&	3.82	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	205	&	2200	&	440	&	3.9	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	205	&	2200	&	440	&	3.86	&	0.05	&	\citet{1976ApJ...208..399M}\\
GJ	205	&	2200	&	440	&	3.9	&	0.05	&	\citet{1989A_A...215..305A}\\
GJ	205	&	2200	&	440	&	3.89	&	0.05	&	\citet{1994PASP..106..508M}\\
GJ	205	&	Johnson	&	K	&	3.9	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	205	&	Johnson	&	K	&	4.03	&	0.05	&	\citet{1971BOTT....6..143I}\\
GJ	205	&	Johnson	&	K	&	3.82	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	205	&	Johnson	&	K	&	3.86	&	0.05	&	\citet{1976ApJ...208..399M}\\
GJ	205	&	3400	&	680	&	3.67	&	0.05	&	\citet{1989A_A...215..305A}\\
GJ	205	&	3500	&	700	&	3.7	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	205	&	3500	&	700	&	3.83	&	0.05	&	\citet{1976ApJ...208..399M}\\
GJ	205	&	Johnson	&	L	&	3.7	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	205	&	Johnson	&	L	&	3.91	&	0.05	&	\citet{1971BOTT....6..143I}\\
GJ	205	&	Johnson	&	L	&	3.83	&	0.05	&	\citet{1976ApJ...208..399M}\\
											
GJ	338A	&	Stromgren	&	u	&	11.53	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	338A	&	Stromgren	&	u	&	11.52	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	338A	&	Stromgren	&	u	&	11.53	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	338A	&	Johnson	&	U	&	10.27	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	338A	&	Johnson	&	U	&	10.37	&	0.05	&	\citet{1976PASP...88..444K}\\
GJ	338A	&	Johnson	&	U	&	10.19	&	0.05	&	\citet{1955ApJS....2..195R}\\
GJ	338A	&	Johnson	&	U	&	10.27	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	338A	&	Stromgren	&	v	&	9.97	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	338A	&	Stromgren	&	v	&	9.96	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	338A	&	Stromgren	&	v	&	9.97	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	338A	&	Johnson	&	B	&	9.07	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	338A	&	Johnson	&	B	&	9.17	&	0.05	&	\citet{1976PASP...88..444K}\\
GJ	338A	&	Johnson	&	B	&	8.98	&	0.05	&	\citet{1955ApJS....2..195R}\\
GJ	338A	&	Johnson	&	B	&	9.05	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	338A	&	Stromgren	&	b	&	8.48	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	338A	&	Stromgren	&	b	&	8.48	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	338A	&	Stromgren	&	b	&	8.48	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	338A	&	Stromgren	&	y	&	7.64	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	338A	&	Stromgren	&	y	&	7.64	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	338A	&	Stromgren	&	y	&	7.64	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	338A	&	Johnson	&	V	&	7.64	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	338A	&	Johnson	&	V	&	7.78	&	0.05	&	\citet{1976PASP...88..444K}\\
GJ	338A	&	Johnson	&	V	&	7.6	&	0.05	&	\citet{1955ApJS....2..195R}\\
GJ	338A	&	Johnson	&	V	&	7.64	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	338A	&	1250	&	250	&	4.91	&	0.05	&	\citet{1991ApJ...368..264A}\\
GJ	338A	&	1250	&	250	&	4.86	&	0.05	&	\citet{1996AJ....112.2238S}\\
GJ	338A	&	2Mass	&	J	&	4.89	&	0.03	&	\citet{2003tmc..book.....C}\\
GJ	338A	&	1650	&	330	&	4.3	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	338A	&	1650	&	330	&	4.25	&	0.05	&	\citet{1991ApJ...368..264A}\\
GJ	338A	&	1650	&	330	&	4.21	&	0.05	&	\citet{1996AJ....112.2238S}\\
GJ	338A	&	2Mass	&	H	&	3.99	&	0.19	&	\citet{2003tmc..book.....C}\\
GJ	338A	&	Johnson	&	H	&	4.25	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	338A	&	2100	&	420	&	4.1	&	0.05	&	\citet{1996AJ....112.2238S}\\
GJ	338A	&	2Mass	&	Ks	&	3.99	&	0.03	&	\citet{2003tmc..book.....C}\\
GJ	338A	&	2200	&	440	&	4.15	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	338A	&	2200	&	440	&	4.09	&	0.05	&	\citet{1991ApJ...368..264A}\\
GJ	338A	&	Johnson	&	K	&	4.09	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	338A	&	3400	&	680	&	3.99	&	0.05	&	\citet{1991ApJ...368..264A}\\
GJ	338A	&	3500	&	700	&	4.1	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	338A	&	Johnson	&	L	&	4	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	338B	&	Geneva	&	U	&	10.95	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	338B	&	Stromgren	&	u	&	11.64	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	338B	&	Stromgren	&	u	&	11.64	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	338B	&	Stromgren	&	u	&	11.65	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	338B	&	Johnson	&	U	&	10.33	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	338B	&	Johnson	&	U	&	10.5	&	0.05	&	\citet{1976PASP...88..444K}\\
GJ	338B	&	Johnson	&	U	&	10.34	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	338B	&	Johnson	&	U	&	10.27	&	0.05	&	\citet{1978A_AS...34....1N}\\
GJ	338B	&	Johnson	&	U	&	10.26	&	0.05	&	\citet{1955ApJS....2..195R}\\
GJ	338B	&	Geneva	&	B1	&	10.03	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	338B	&	Stromgren	&	v	&	10.08	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	338B	&	Stromgren	&	v	&	10.08	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	338B	&	Stromgren	&	v	&	10.08	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	338B	&	Geneva	&	B	&	8.57	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	338B	&	Geneva	&	B2	&	9.59	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	338B	&	Johnson	&	B	&	9.16	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	338B	&	Johnson	&	B	&	9.1	&	0.05	&	\citet{1976PASP...88..444K}\\
GJ	338B	&	Johnson	&	B	&	9.09	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	338B	&	Johnson	&	B	&	9.07	&	0.05	&	\citet{1978A_AS...34....1N}\\
GJ	338B	&	Johnson	&	B	&	9.04	&	0.05	&	\citet{1955ApJS....2..195R}\\
GJ	338B	&	Stromgren	&	b	&	8.6	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	338B	&	Stromgren	&	b	&	8.6	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	338B	&	Stromgren	&	b	&	8.6	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	338B	&	Geneva	&	V1	&	8.6	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	338B	&	Stromgren	&	y	&	7.74	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	338B	&	Stromgren	&	y	&	7.74	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	338B	&	Stromgren	&	y	&	7.74	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	338B	&	Geneva	&	V	&	7.77	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	338B	&	Johnson	&	V	&	7.74	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	338B	&	Johnson	&	V	&	7.66	&	0.05	&	\citet{1976PASP...88..444K}\\
GJ	338B	&	Johnson	&	V	&	7.67	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	338B	&	Johnson	&	V	&	7.71	&	0.05	&	\citet{1978A_AS...34....1N}\\
GJ	338B	&	Johnson	&	V	&	7.7	&	0.05	&	\citet{1955ApJS....2..195R}\\
GJ	338B	&	Geneva	&	G	&	8.56	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	338B	&	1250	&	250	&	4.96	&	0.05	&	\citet{1991ApJ...368..264A}\\
GJ	338B	&	2Mass	&	J	&	4.78	&	0.17	&	\citet{2003tmc..book.....C}\\
GJ	338B	&	1650	&	330	&	4.25	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	338B	&	1650	&	330	&	4.3	&	0.05	&	\citet{1991ApJ...368..264A}\\
GJ	338B	&	2Mass	&	H	&	4.04	&	0.21	&	\citet{2003tmc..book.....C}\\
GJ	338B	&	Johnson	&	H	&	4.3	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	338B	&	2Mass	&	Ks	&	4.14	&	0.01	&	\citet{2003tmc..book.....C}\\
GJ	338B	&	2200	&	440	&	4.09	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	338B	&	2200	&	440	&	4.13	&	0.05	&	\citet{1991ApJ...368..264A}\\
GJ	338B	&	Johnson	&	K	&	4.15	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	338B	&	3400	&	680	&	4.02	&	0.05	&	\citet{1991ApJ...368..264A}\\
GJ	338B	&	3500	&	700	&	4	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	338B	&	Johnson	&	L	&	4.1	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	380	&	Johnson	&	U	&	9.23	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	380	&	Geneva	&	B1	&	8.83	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	380	&	Stromgren	&	v	&	8.93	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	380	&	Stromgren	&	v	&	8.93	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	380	&	Stromgren	&	v	&	8.93	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	380	&	Stromgren	&	v	&	8.9	&	0.08	&	\citet{1966GeoOM..21....0C}\\
GJ	380	&	Geneva	&	B	&	7.33	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	380	&	Geneva	&	B2	&	8.34	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	380	&	Johnson	&	B	&	7.97	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	380	&	Johnson	&	B	&	7.98	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	380	&	Johnson	&	B	&	8.04	&	0.05	&	\citet{1963ArA.....3..273O}\\
GJ	380	&	Johnson	&	B	&	7.97	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	380	&	Johnson	&	B	&	7.94	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	380	&	Johnson	&	B	&	7.98	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	380	&	Johnson	&	B	&	7.94	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	380	&	Johnson	&	B	&	7.94	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	380	&	Stromgren	&	b	&	7.4	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	380	&	Stromgren	&	b	&	7.4	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	380	&	Stromgren	&	b	&	7.4	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	380	&	Stromgren	&	b	&	7.41	&	0.08	&	\citet{1966GeoOM..21....0C}\\
GJ	380	&	Geneva	&	V1	&	7.41	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	380	&	Stromgren	&	y	&	6.61	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	380	&	Stromgren	&	y	&	6.61	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	380	&	Stromgren	&	y	&	6.61	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	380	&	Stromgren	&	y	&	6.61	&	0.08	&	\citet{1966GeoOM..21....0C}\\
GJ	380	&	Geneva	&	V	&	6.58	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	380	&	Johnson	&	V	&	6.59	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	380	&	Johnson	&	V	&	6.6	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	380	&	Johnson	&	V	&	6.66	&	0.05	&	\citet{1963ArA.....3..273O}\\
GJ	380	&	Johnson	&	V	&	6.6	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	380	&	Johnson	&	V	&	6.6	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	380	&	Johnson	&	V	&	6.6	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	380	&	Johnson	&	V	&	6.59	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	380	&	Johnson	&	V	&	6.59	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	380	&	Geneva	&	G	&	7.38	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	380	&	1250	&	250	&	4.1	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	380	&	1250	&	250	&	3.97	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	380	&	1250	&	250	&	3.98	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	380	&	1250	&	250	&	4.02	&	0.05	&	\citet{1977AJ.....82..729P}\\
GJ	380	&	2Mass	&	J	&	3.89	&	0.29	&	\citet{2003tmc..book.....C}\\
GJ	380	&	Johnson	&	J	&	4.1	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	380	&	Johnson	&	J	&	3.98	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	380	&	Johnson	&	J	&	3.97	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	380	&	1650	&	330	&	3.27	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	380	&	1650	&	330	&	3.37	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	380	&	1650	&	330	&	3.32	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	380	&	1650	&	330	&	3.34	&	0.05	&	\citet{1977AJ.....82..729P}\\
GJ	380	&	2Mass	&	H	&	3.3	&	0.26	&	\citet{2003tmc..book.....C}\\
GJ	380	&	Johnson	&	H	&	3.32	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	380	&	Johnson	&	H	&	3.37	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	380	&	Johnson	&	H	&	3.27	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	380	&	2Mass	&	Ks	&	2.96	&	0.29	&	\citet{2003tmc..book.....C}\\
GJ	380	&	2200	&	440	&	3.26	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	380	&	2200	&	440	&	3.15	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	380	&	2200	&	440	&	3.23	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	380	&	2200	&	440	&	3.19	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	380	&	2200	&	440	&	3.21	&	0.05	&	\citet{1977AJ.....82..729P}\\
GJ	380	&	Johnson	&	K	&	3.26	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	380	&	Johnson	&	K	&	3.19	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	380	&	Johnson	&	K	&	3.23	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	380	&	Johnson	&	K	&	3.15	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	380	&	3400	&	680	&	3.06	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	380	&	3400	&	680	&	3.11	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	380	&	3500	&	700	&	3.01	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	380	&	3500	&	700	&	3.1	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	380	&	Johnson	&	L	&	3.06	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	380	&	Johnson	&	L	&	3.11	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	380	&	Johnson	&	L	&	3.1	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	380	&	Johnson	&	L	&	3.01	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	411	&	Stromgren	&	u	&	11.42	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	411	&	Stromgren	&	u	&	11.42	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	411	&	Stromgren	&	u	&	11.43	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	411	&	Johnson	&	U	&	10.11	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	411	&	Johnson	&	U	&	10.15	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	411	&	Johnson	&	U	&	10.16	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	411	&	Johnson	&	U	&	10.04	&	0.05	&	\citet{1985A_AS...61..331O}\\
GJ	411	&	Johnson	&	U	&	10.13	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	411	&	Johnson	&	U	&	10.13	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	411	&	Johnson	&	U	&	10.12	&	0.05	&	\citet{1964BOTT....3..305J}\\
GJ	411	&	Stromgren	&	v	&	9.87	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	411	&	Stromgren	&	v	&	9.88	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	411	&	Stromgren	&	v	&	9.87	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	411	&	Johnson	&	B	&	8.98	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	411	&	Johnson	&	B	&	9.01	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	411	&	Johnson	&	B	&	9.01	&	0.05	&	\citet{1963ArA.....3..273O}\\
GJ	411	&	Johnson	&	B	&	9.01	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	411	&	Johnson	&	B	&	8.98	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	411	&	Johnson	&	B	&	8.96	&	0.05	&	\citet{1985A_AS...61..331O}\\
GJ	411	&	Johnson	&	B	&	9.01	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	411	&	Johnson	&	B	&	9.01	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	411	&	Johnson	&	B	&	9	&	0.05	&	\citet{1964BOTT....3..305J}\\
GJ	411	&	Stromgren	&	b	&	8.47	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	411	&	Stromgren	&	b	&	8.47	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	411	&	Stromgren	&	b	&	8.47	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	411	&	Stromgren	&	y	&	7.49	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	411	&	Stromgren	&	y	&	7.49	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	411	&	Stromgren	&	y	&	7.49	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	411	&	Johnson	&	V	&	7.47	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	411	&	Johnson	&	V	&	7.5	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	411	&	Johnson	&	V	&	7.51	&	0.05	&	\citet{1963ArA.....3..273O}\\
GJ	411	&	Johnson	&	V	&	7.48	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	411	&	Johnson	&	V	&	7.48	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	411	&	Johnson	&	V	&	7.52	&	0.05	&	\citet{1985A_AS...61..331O}\\
GJ	411	&	Johnson	&	V	&	7.5	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	411	&	Johnson	&	V	&	7.5	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	411	&	Johnson	&	V	&	7.49	&	0.05	&	\citet{1964BOTT....3..305J}\\
GJ	411	&	1250	&	250	&	4.09	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	411	&	1250	&	250	&	4.13	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	411	&	1250	&	250	&	4.16	&	0.05	&	\citet{1977AJ.....82..729P}\\
GJ	411	&	1250	&	250	&	4.1	&	0.05	&	\citet{1986ApJS...61..531S}\\
GJ	411	&	1250	&	250	&	4.13	&	0.05	&	\citet{1987MNRAS.227..315B}\\
GJ	411	&	1250	&	250	&	4.13	&	0.05	&	\citet{1991ApJ...368..264A}\\
GJ	411	&	1250	&	250	&	4.04	&	0.05	&	\citet{1996AJ....112.2238S}\\
GJ	411	&	2Mass	&	J	&	4.2	&	0.24	&	\citet{2003tmc..book.....C}\\
GJ	411	&	Johnson	&	J	&	4.09	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	411	&	Johnson	&	J	&	4.1	&	0.05	&	\citet{1964BOTT....3..305J}\\
GJ	411	&	Johnson	&	J	&	4.13	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	411	&	1280	&	256	&	4.1	&	0.05	&	\citet{1994A_AS..107..365A}\\
GJ	411	&	1650	&	330	&	3.59	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	411	&	1650	&	330	&	3.56	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	411	&	1650	&	330	&	3.57	&	0.05	&	\citet{1977AJ.....82..729P}\\
GJ	411	&	1650	&	330	&	3.56	&	0.05	&	\citet{1986ApJS...61..531S}\\
GJ	411	&	1650	&	330	&	3.56	&	0.05	&	\citet{1991ApJ...368..264A}\\
GJ	411	&	1650	&	330	&	3.56	&	0.05	&	\citet{1994A_AS..107..365A}\\
GJ	411	&	1650	&	330	&	3.57	&	0.05	&	\citet{1996AJ....112.2238S}\\
GJ	411	&	2Mass	&	H	&	3.64	&	0.2	&	\citet{2003tmc..book.....C}\\
GJ	411	&	Johnson	&	H	&	3.56	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	411	&	Johnson	&	H	&	3.59	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	411	&	2100	&	420	&	3.39	&	0.05	&	\citet{1996AJ....112.2238S}\\
GJ	411	&	2Mass	&	Ks	&	3.25	&	0.31	&	\citet{2003tmc..book.....C}\\
GJ	411	&	2190	&	438	&	3.34	&	0.05	&	\citet{1994A_AS..107..365A}\\
GJ	411	&	2200	&	440	&	3.34	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	411	&	2200	&	440	&	3.38	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	411	&	2200	&	440	&	3.35	&	0.05	&	\citet{1986ApJS...61..531S}\\
GJ	411	&	2200	&	440	&	3.34	&	0.05	&	\citet{1991ApJ...368..264A}\\
GJ	411	&	2200	&	440	&	3.35	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	411	&	2200	&	440	&	3.37	&	0.05	&	\citet{1977AJ.....82..729P}\\
GJ	411	&	Johnson	&	K	&	3.34	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	411	&	Johnson	&	K	&	3.31	&	0.05	&	\citet{1964BOTT....3..305J}\\
GJ	411	&	Johnson	&	K	&	3.35	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	411	&	Johnson	&	K	&	3.38	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	411	&	2300	&	460	&	3.38	&	0.05	&	\citet{1974PASP...86..989B}\\
GJ	411	&	3400	&	680	&	3.17	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	411	&	3400	&	680	&	3.2	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	411	&	3400	&	680	&	3.15	&	0.05	&	\citet{1991ApJ...368..264A}\\
GJ	411	&	3500	&	700	&	3.09	&	0.05	&	\citet{1971ApJ...165..285G}\\
GJ	411	&	3500	&	700	&	3.2	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	411	&	Johnson	&	L	&	3.17	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	411	&	Johnson	&	L	&	3.08	&	0.05	&	\citet{1964BOTT....3..305J}\\
GJ	411	&	Johnson	&	L	&	3.2	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	411	&	Johnson	&	L	&	3.2	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	412A	&	Geneva	&	U	&	12.1	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	412A	&	Johnson	&	U	&	11.38	&	0.05	&	\citet{1978A_AS...34....1N}\\
GJ	412A	&	Johnson	&	U	&	11.34	&	0.05	&	\citet{1955ApJS....2..195R}\\
GJ	412A	&	Johnson	&	U	&	11.44	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	412A	&	Johnson	&	U	&	11.51	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	412A	&	Geneva	&	B1	&	11.17	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	412A	&	Geneva	&	B	&	9.73	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	412A	&	Geneva	&	B2	&	10.77	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	412A	&	Johnson	&	B	&	10.22	&	0.05	&	\citet{1978A_AS...34....1N}\\
GJ	412A	&	Johnson	&	B	&	10.32	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	412A	&	Johnson	&	B	&	10.18	&	0.05	&	\citet{1955ApJS....2..195R}\\
GJ	412A	&	Johnson	&	B	&	10.26	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	412A	&	Johnson	&	B	&	10.31	&	0.05	&	\citet{1977ApJ...215..845W}\\
GJ	412A	&	Johnson	&	B	&	10.32	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	412A	&	Geneva	&	V1	&	9.62	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	412A	&	Geneva	&	V	&	8.8	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	412A	&	Johnson	&	V	&	8.68	&	0.05	&	\citet{1978A_AS...34....1N}\\
GJ	412A	&	Johnson	&	V	&	8.74	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	412A	&	Johnson	&	V	&	8.66	&	0.05	&	\citet{1955ApJS....2..195R}\\
GJ	412A	&	Johnson	&	V	&	8.74	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	412A	&	Johnson	&	V	&	8.77	&	0.05	&	\citet{1977ApJ...215..845W}\\
GJ	412A	&	Johnson	&	V	&	8.77	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	412A	&	Geneva	&	G	&	9.6	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	412A	&	1250	&	250	&	5.64	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	412A	&	1250	&	250	&	5.56	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	412A	&	1250	&	250	&	5.62	&	0.05	&	\citet{1977AJ.....82..729P}\\
GJ	412A	&	1250	&	250	&	5.54	&	0.05	&	\citet{1986ApJS...61..531S}\\
GJ	412A	&	Johnson	&	J	&	5.64	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	412A	&	Johnson	&	J	&	5.56	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	412A	&	1650	&	330	&	4.95	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	412A	&	1650	&	330	&	4.95	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	412A	&	1650	&	330	&	4.99	&	0.05	&	\citet{1977AJ.....82..729P}\\
GJ	412A	&	1650	&	330	&	4.97	&	0.05	&	\citet{1986ApJS...61..531S}\\
GJ	412A	&	Johnson	&	H	&	4.95	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	412A	&	Johnson	&	H	&	4.95	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	412A	&	2200	&	440	&	4.74	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	412A	&	2200	&	440	&	4.71	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	412A	&	2200	&	440	&	4.76	&	0.05	&	\citet{1986ApJS...61..531S}\\
GJ	412A	&	2200	&	440	&	4.76	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	412A	&	2200	&	440	&	4.8	&	0.05	&	\citet{1977AJ.....82..729P}\\
GJ	412A	&	Johnson	&	K	&	4.74	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	412A	&	Johnson	&	K	&	4.71	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	412A	&	Johnson	&	K	&	4.76	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	412A	&	3400	&	680	&	4.5	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	412A	&	3400	&	680	&	4.6	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	412A	&	3500	&	700	&	4.6	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	412A	&	Johnson	&	L	&	4.5	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	412A	&	Johnson	&	L	&	4.6	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	412A	&	Johnson	&	L	&	4.6	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	436	&	Geneva	&	U	&	14.03	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	436	&	Geneva	&	U	&	14.04	&	0.1	&	\citet{1972VA.....14...13G}\\
GJ	436	&	Johnson	&	U	&	13.38	&	0.05	&	\citet{1991PASP..103..973D}\\
GJ	436	&	Johnson	&	U	&	13.43	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	436	&	Geneva	&	B1	&	12.97	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	436	&	Geneva	&	B1	&	12.97	&	0.1	&	\citet{1972VA.....14...13G}\\
GJ	436	&	Geneva	&	B	&	11.58	&	0.1	&	\citet{1972VA.....14...13G}\\
GJ	436	&	Johnson	&	B	&	12.17	&	0.05	&	\citet{1993AJ....105.1962W}\\
GJ	436	&	Johnson	&	B	&	12.19	&	0.05	&	\citet{1991PASP..103..973D}\\
GJ	436	&	Johnson	&	B	&	12.2	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	436	&	Geneva	&	B2	&	12.64	&	0.1	&	\citet{1972VA.....14...13G}\\
GJ	436	&	Geneva	&	B2	&	12.64	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	436	&	Geneva	&	V1	&	11.47	&	0.1	&	\citet{1972VA.....14...13G}\\
GJ	436	&	Geneva	&	V1	&	11.47	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	436	&	Geneva	&	V	&	10.66	&	0.1	&	\citet{1972VA.....14...13G}\\
GJ	436	&	Geneva	&	V	&	10.67	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	436	&	Johnson	&	V	&	10.65	&	0.05	&	\citet{1993AJ....105.1962W}\\
GJ	436	&	Johnson	&	V	&	10.68	&	0.05	&	\citet{1991PASP..103..973D}\\
GJ	436	&	Johnson	&	V	&	10.68	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	436	&	Geneva	&	G	&	11.55	&	0.1	&	\citet{1972VA.....14...13G}\\
GJ	436	&	Geneva	&	G	&	11.55	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	436	&	Cousins	&	Rc	&	9.34	&	0.05	&	\citet{1993AJ....105.1962W}\\
GJ	436	&	Cousins	&	Ic	&	8.38	&	0.05	&	\citet{1993AJ....105.1962W}\\
GJ	436	&	2Mass	&	J	&	6.9	&	0.02	&	\citet{2003tmc..book.....C}\\
GJ	436	&	2Mass	&	H	&	6.32	&	0.02	&	\citet{2003tmc..book.....C}\\
GJ	436	&	2Mass	&	Ks	&	6.07	&	0.01	&	\citet{2003tmc..book.....C}\\
GJ	526	&	Geneva	&	U	&	11.58	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	526	&	Stromgren	&	u	&	12.45	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	526	&	Stromgren	&	u	&	12.45	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	526	&	Johnson	&	U	&	10.95	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	526	&	Johnson	&	U	&	11.02	&	0.05	&	\citet{1955ApJS....2..195R}\\
GJ	526	&	Johnson	&	U	&	11.01	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	526	&	Johnson	&	U	&	11.02	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	526	&	Geneva	&	B1	&	10.66	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	526	&	Stromgren	&	v	&	10.73	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	526	&	Stromgren	&	v	&	10.73	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	526	&	Geneva	&	B	&	9.28	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	526	&	Geneva	&	B2	&	10.35	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	526	&	Johnson	&	B	&	9.91	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	526	&	Johnson	&	B	&	9.91	&	0.05	&	\citet{1955ApJS....2..195R}\\
GJ	526	&	Johnson	&	B	&	9.94	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	526	&	Johnson	&	B	&	9.9	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	526	&	Johnson	&	B	&	9.93	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	526	&	Stromgren	&	b	&	9.43	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	526	&	Stromgren	&	b	&	9.43	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	526	&	Geneva	&	V1	&	9.28	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	526	&	Stromgren	&	y	&	8.46	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	526	&	Stromgren	&	y	&	8.46	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	526	&	Geneva	&	V	&	8.47	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	526	&	Johnson	&	V	&	8.43	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	526	&	Johnson	&	V	&	8.47	&	0.05	&	\citet{1955ApJS....2..195R}\\
GJ	526	&	Johnson	&	V	&	8.47	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	526	&	Johnson	&	V	&	8.46	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	526	&	Johnson	&	V	&	8.5	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	526	&	Geneva	&	G	&	9.31	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	526	&	1250	&	250	&	5.34	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	526	&	1250	&	250	&	5.26	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	526	&	1250	&	250	&	5.24	&	0.05	&	\citet{1986ApJS...61..531S}\\
GJ	526	&	1250	&	250	&	5.23	&	0.05	&	\citet{1996AJ....112.2238S}\\
GJ	526	&	Johnson	&	J	&	5.26	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	526	&	Johnson	&	J	&	5.34	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	526	&	1650	&	330	&	4.66	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	526	&	1650	&	330	&	4.64	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	526	&	1650	&	330	&	4.66	&	0.05	&	\citet{1986ApJS...61..531S}\\
GJ	526	&	1650	&	330	&	4.65	&	0.05	&	\citet{1996AJ....112.2238S}\\
GJ	526	&	Johnson	&	H	&	4.64	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	526	&	Johnson	&	H	&	4.66	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	526	&	2100	&	420	&	4.48	&	0.05	&	\citet{1996AJ....112.2238S}\\
GJ	526	&	2200	&	440	&	4.44	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	526	&	2200	&	440	&	4.47	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	526	&	2200	&	440	&	4.46	&	0.05	&	\citet{1986ApJS...61..531S}\\
GJ	526	&	2200	&	440	&	4.46	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	526	&	Johnson	&	K	&	4.46	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	526	&	Johnson	&	K	&	4.47	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	526	&	Johnson	&	K	&	4.44	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	526	&	3400	&	680	&	4.38	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	526	&	3400	&	680	&	4.33	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	526	&	3500	&	700	&	4.2	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	526	&	Johnson	&	L	&	4.33	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	526	&	Johnson	&	L	&	4.2	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	526	&	Johnson	&	L	&	4.38	&	0.05	&	\citet{1965ApJ...141..170J}\\
											
											
GJ	570A	&	Stromgren	&	u	&	9.07	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	570A	&	Stromgren	&	u	&	9.09	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	570A	&	Stromgren	&	u	&	9.12	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	570A	&	Stromgren	&	u	&	9.18	&	0.08	&	\citet{1984A_AS...57..443O}\\
GJ	570A	&	Johnson	&	U	&	7.88	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	570A	&	Johnson	&	U	&	7.89	&	0.1	&	\citet{1972MNSSA..31...75C}\\
GJ	570A	&	Johnson	&	U	&	7.94	&	0.1	&	\citet{1965ApJ...141..170J}\\
GJ	570A	&	Johnson	&	U	&	7.96	&	0.1	&	\citet{1986EgUBV........0M}\\
GJ	570A	&	Johnson	&	U	&	7.97	&	0.1	&	\citet{1957ApJ...126..113J}\\
GJ	570A	&	Johnson	&	U	&	7.98	&	0.1	&	\citet{1967AJ.....72.1334C}\\
GJ	570A	&	Stromgren	&	v	&	7.62	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	570A	&	Stromgren	&	v	&	7.63	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	570A	&	Stromgren	&	v	&	7.64	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	570A	&	Stromgren	&	v	&	7.68	&	0.08	&	\citet{1984A_AS...57..443O}\\
GJ	570A	&	Johnson	&	B	&	6.82	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	570A	&	Johnson	&	B	&	6.84	&	0.1	&	\citet{1972MNSSA..31...75C}\\
GJ	570A	&	Johnson	&	B	&	6.88	&	0.1	&	\citet{1965ApJ...141..170J}\\
GJ	570A	&	Johnson	&	B	&	6.9	&	0.1	&	\citet{1986EgUBV........0M}\\
GJ	570A	&	Johnson	&	B	&	6.91	&	0.1	&	\citet{1957ApJ...126..113J}\\
GJ	570A	&	Johnson	&	B	&	6.91	&	0.1	&	\citet{1967AJ.....72.1334C}\\
GJ	570A	&	Stromgren	&	b	&	6.35	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	570A	&	Stromgren	&	b	&	6.36	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	570A	&	Stromgren	&	b	&	6.37	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	570A	&	Stromgren	&	b	&	6.37	&	0.08	&	\citet{1984A_AS...57..443O}\\
GJ	570A	&	Stromgren	&	y	&	5.74	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	570A	&	Stromgren	&	y	&	5.74	&	0.08	&	\citet{1984A_AS...57..443O}\\
GJ	570A	&	Stromgren	&	y	&	5.74	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	570A	&	Stromgren	&	y	&	5.74	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	570A	&	Johnson	&	V	&	5.71	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	570A	&	Johnson	&	V	&	5.73	&	0.05	&	\citet{1972MNSSA..31...75C}\\
GJ	570A	&	Johnson	&	V	&	5.78	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	570A	&	Johnson	&	V	&	5.78	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	570A	&	Johnson	&	V	&	5.8	&	0.05	&	\citet{1957ApJ...126..113J}\\
GJ	570A	&	Johnson	&	V	&	5.8	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	570A	&	1250	&	250	&	3.83	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	570A	&	1250	&	250	&	3.83	&	0.05	&	\citet{1989A_A...215..305A}\\
GJ	570A	&	1250	&	250	&	3.84	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	570A	&	1250	&	250	&	3.84	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	570A	&	1250	&	250	&	3.82	&	0.05	&	\citet{1976ApJ...208..399M}\\
GJ	570A	&	1280	&	256	&	3.77	&	0.05	&	\citet{1994A_AS..107..365A}\\
GJ	570A	&	1650	&	330	&	3.23	&	0.05	&	\citet{1989A_A...215..305A}\\
GJ	570A	&	1650	&	330	&	3.26	&	0.05	&	\citet{1994A_AS..107..365A}\\
GJ	570A	&	1650	&	330	&	3.27	&	0.05	&	\citet{1976ApJ...208..399M}\\
GJ	570A	&	2190	&	438	&	3.15	&	0.05	&	\citet{1994A_AS..107..365A}\\
GJ	570A	&	2200	&	440	&	3.06	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	570A	&	2200	&	440	&	3.06	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	570A	&	2200	&	440	&	3.06	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	570A	&	2200	&	440	&	3.19	&	0.05	&	\citet{1989A_A...215..305A}\\
GJ	570A	&	2200	&	440	&	3.15	&	0.05	&	\citet{1976ApJ...208..399M}\\
GJ	570A	&	Johnson	&	K	&	2.75	&	0.1	&	\citet{1969tmss.book.....N}\\
GJ	570A	&	3400	&	680	&	2.79	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	570A	&	3400	&	680	&	2.85	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	570A	&	3400	&	680	&	3.06	&	0.05	&	\citet{1989A_A...215..305A}\\
GJ	570A	&	3500	&	700	&	2.79	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	570A	&	3500	&	700	&	3.11	&	0.05	&	\citet{1976ApJ...208..399M}\\
GJ	581	&	Johnson	&	U	&	13.4	&	0.5	&	\citet{2010MNRAS.403.1949K}\\
GJ	581	&	Johnson	&	B	&	12.17	&	0.11	&	\citet{2010MNRAS.403.1949K}\\
GJ	581	&	Johnson	&	B	&	12.17	&	0.05	&	\citet{2009ApJS..185..289R}\\
GJ	581	&	Johnson	&	B	&	12.19	&	0.05	&	\citet{1990A_AS...83..357B}\\
GJ	581	&	Johnson	&	V	&	10.57	&	0.05	&	\citet{1990A_AS...83..357B}\\
GJ	581	&	Johnson	&	V	&	10.57	&	0.05	&	\citet{2009ApJS..185..289R}\\
GJ	581	&	Cousins	&	Rc	&	9.47	&	0.05	&	\citet{1990A_AS...83..357B}\\
GJ	581	&	Cousins	&	Ic	&	8.04	&	0.05	&	\citet{2009A_A...499..129L}\\
GJ	581	&	Cousins	&	Ic	&	8.06	&	0.05	&	\citet{1990A_AS...83..357B}\\
GJ	581	&	2MASS	&	J	&	6.69	&	0.03	&	\citet{2007MNRAS.380.1261K}\\
GJ	581	&	2MASS	&	J	&	6.69	&	0.03	&	\citet{2010MNRAS.403.1949K}\\
GJ	581	&	2Mass	&	J	&	6.71	&	0.02	&	\citet{2003tmc..book.....C}\\
GJ	581	&	2Mass	&	H	&	6.1	&	0.03	&	\citet{2003tmc..book.....C}\\
GJ	581	&	2MASS	&	H	&	6.12	&	0.04	&	\citet{2007MNRAS.380.1261K}\\
GJ	581	&	2MASS	&	H	&	6.13	&	0.03	&	\citet{2010MNRAS.403.1949K}\\
GJ	581	&	2Mass	&	Ks	&	5.84	&	0.02	&	\citet{2003tmc..book.....C}\\
GJ	581	&	2MASS	&	Ks	&	5.85	&	0.03	&	\citet{2010MNRAS.403.1949K}\\
GJ	581	&	2MASS	&	Ks	&	5.85	&	0.03	&	\citet{2007MNRAS.380.1261K}\\
GJ	631	&	Stromgren	&	u	&	8.26	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	631	&	Stromgren	&	u	&	8.24	&	0.08	&	\citet{1977A_AS...29..313O}\\
GJ	631	&	Stromgren	&	u	&	8.26	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	631	&	Stromgren	&	u	&	8.26	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	631	&	Stromgren	&	u	&	8.27	&	0.08	&	\citet{1994A_AS..104..429O}\\
GJ	631	&	Stromgren	&	u	&	8.28	&	0.08	&	\citet{1984A_AS...57..443O}\\
GJ	631	&	Johnson	&	U	&	7.16	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	631	&	Johnson	&	U	&	7	&	0.05	&	\citet{1971PASP...83...79F}\\
GJ	631	&	Johnson	&	U	&	6.99	&	0.05	&	\citet{1969AcA....19..229R}\\
GJ	631	&	Johnson	&	U	&	7.12	&	0.05	&	\citet{1979A_AS...36..297B}\\
GJ	631	&	Johnson	&	U	&	7	&	0.05	&	\citet{1957ApJ...126..113J}\\
GJ	631	&	Johnson	&	U	&	7.13	&	0.05	&	\citet{1963MNSSA..22...12C}\\
GJ	631	&	Johnson	&	U	&	7.1	&	0.05	&	\citet{1984SAAOC...8...59C}\\
GJ	631	&	Johnson	&	U	&	7.08	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	631	&	Johnson	&	U	&	7	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	631	&	Stromgren	&	v	&	7.11	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	631	&	Stromgren	&	v	&	7.09	&	0.08	&	\citet{1977A_AS...29..313O}\\
GJ	631	&	Stromgren	&	v	&	7.11	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	631	&	Stromgren	&	v	&	7.11	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	631	&	Stromgren	&	v	&	7.11	&	0.08	&	\citet{1994A_AS..104..429O}\\
GJ	631	&	Stromgren	&	v	&	7.12	&	0.08	&	\citet{1984A_AS...57..443O}\\
GJ	631	&	Johnson	&	B	&	6.65	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	631	&	Johnson	&	B	&	6.55	&	0.05	&	\citet{1971PASP...83...79F}\\
GJ	631	&	Johnson	&	B	&	6.56	&	0.05	&	\citet{1969AcA....19..229R}\\
GJ	631	&	Johnson	&	B	&	6.62	&	0.05	&	\citet{1979A_AS...36..297B}\\
GJ	631	&	Johnson	&	B	&	6.55	&	0.05	&	\citet{1957ApJ...126..113J}\\
GJ	631	&	Johnson	&	B	&	6.6	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	631	&	Johnson	&	B	&	6.57	&	0.05	&	\citet{1963MNSSA..22...12C}\\
GJ	631	&	Johnson	&	B	&	6.6	&	0.05	&	\citet{1984SAAOC...8...59C}\\
GJ	631	&	Johnson	&	B	&	6.58	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	631	&	Johnson	&	B	&	6.55	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	631	&	Stromgren	&	b	&	6.25	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	631	&	Stromgren	&	b	&	6.25	&	0.08	&	\citet{1977A_AS...29..313O}\\
GJ	631	&	Stromgren	&	b	&	6.25	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	631	&	Stromgren	&	b	&	6.25	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	631	&	Stromgren	&	b	&	6.25	&	0.08	&	\citet{1994A_AS..104..429O}\\
GJ	631	&	Stromgren	&	b	&	6.25	&	0.08	&	\citet{1984A_AS...57..443O}\\
GJ	631	&	Stromgren	&	y	&	5.76	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	631	&	Stromgren	&	y	&	5.76	&	0.08	&	\citet{1977A_AS...29..313O}\\
GJ	631	&	Stromgren	&	y	&	5.76	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	631	&	Stromgren	&	y	&	5.76	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	631	&	Stromgren	&	y	&	5.76	&	0.08	&	\citet{1994A_AS..104..429O}\\
GJ	631	&	Stromgren	&	y	&	5.76	&	0.08	&	\citet{1984A_AS...57..443O}\\
GJ	631	&	Johnson	&	V	&	5.8	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	631	&	Johnson	&	V	&	5.74	&	0.05	&	\citet{1971PASP...83...79F}\\
GJ	631	&	Johnson	&	V	&	5.74	&	0.05	&	\citet{1969AcA....19..229R}\\
GJ	631	&	Johnson	&	V	&	5.78	&	0.05	&	\citet{1979A_AS...36..297B}\\
GJ	631	&	Johnson	&	V	&	5.74	&	0.05	&	\citet{1957ApJ...126..113J}\\
GJ	631	&	Johnson	&	V	&	5.78	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	631	&	Johnson	&	V	&	5.75	&	0.05	&	\citet{1963MNSSA..22...12C}\\
GJ	631	&	Johnson	&	V	&	5.77	&	0.05	&	\citet{1984SAAOC...8...59C}\\
GJ	631	&	Johnson	&	V	&	5.76	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	631	&	Johnson	&	V	&	5.74	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	631	&	Johnson	&	R	&	5.13	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	631	&	Johnson	&	I	&	4.74	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	631	&	2Mass	&	J	&	4.45	&	0.28	&	\citet{2003tmc..book.....C}\\
GJ	631	&	Johnson	&	J	&	4.32	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	631	&	2Mass	&	H	&	4.05	&	0.21	&	\citet{2003tmc..book.....C}\\
GJ	631	&	Johnson	&	H	&	3.86	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	631	&	2Mass	&	Ks	&	4.04	&	0.23	&	\citet{2003tmc..book.....C}\\
GJ	631	&	Johnson	&	K	&	3.83	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	631	&	Johnson	&	L	&	3.8	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	687	&	Geneva	&	U	&	12.4	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	687	&	Johnson	&	U	&	11.73	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	687	&	Johnson	&	U	&	11.76	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	687	&	Geneva	&	B1	&	11.38	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	687	&	Geneva	&	B	&	10.03	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	687	&	Geneva	&	B2	&	11.11	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	687	&	Johnson	&	B	&	10.65	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	687	&	Johnson	&	B	&	10.66	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	687	&	Johnson	&	B	&	10.72	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	687	&	Geneva	&	V1	&	9.94	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	687	&	Geneva	&	V	&	9.16	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	687	&	Johnson	&	V	&	9.15	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	687	&	Johnson	&	V	&	9.12	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	687	&	Johnson	&	V	&	9.22	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	687	&	Geneva	&	G	&	10.08	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	687	&	1250	&	250	&	5.37	&	0.05	&	\citet{1977AJ.....82..729P}\\
GJ	687	&	1250	&	250	&	5.32	&	0.05	&	\citet{1986ApJS...61..531S}\\
GJ	687	&	1250	&	250	&	5.32	&	0.05	&	\citet{1991ApJ...368..264A}\\
GJ	687	&	2Mass	&	J	&	5.34	&	0.01	&	\citet{2003tmc..book.....C}\\
GJ	687	&	1650	&	330	&	4.78	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	687	&	1650	&	330	&	4.75	&	0.05	&	\citet{1977AJ.....82..729P}\\
GJ	687	&	1650	&	330	&	4.74	&	0.05	&	\citet{1986ApJS...61..531S}\\
GJ	687	&	1650	&	330	&	4.74	&	0.05	&	\citet{1991ApJ...368..264A}\\
GJ	687	&	2Mass	&	H	&	4.77	&	0.03	&	\citet{2003tmc..book.....C}\\
GJ	687	&	Johnson	&	H	&	4.78	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	687	&	2Mass	&	Ks	&	4.55	&	0.02	&	\citet{2003tmc..book.....C}\\
GJ	687	&	2200	&	440	&	4.55	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	687	&	2200	&	440	&	4.52	&	0.05	&	\citet{1986ApJS...61..531S}\\
GJ	687	&	2200	&	440	&	4.51	&	0.05	&	\citet{1991ApJ...368..264A}\\
GJ	687	&	2200	&	440	&	4.54	&	0.05	&	\citet{1977AJ.....82..729P}\\
GJ	687	&	Johnson	&	K	&	4.55	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	687	&	2300	&	460	&	4.57	&	0.05	&	\citet{1974PASP...86..989B}\\
GJ	687	&	3400	&	680	&	4.31	&	0.05	&	\citet{1991ApJ...368..264A}\\
GJ	687	&	3500	&	700	&	4.3	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	687	&	Johnson	&	L	&	4.3	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	699	&	Johnson	&	U	&	12.57	&	0.05	&	\citet{1978A_AS...34....1N}\\
GJ	699	&	Johnson	&	U	&	12.59	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	699	&	Johnson	&	U	&	12.55	&	0.05	&	\citet{1983AJ.....88..439L}\\
GJ	699	&	Johnson	&	U	&	12.48	&	0.05	&	\citet{1973PASP...85..721U}\\
GJ	699	&	Johnson	&	U	&	12.45	&	0.05	&	\citet{1976PUSNO..24c...1D}\\
GJ	699	&	Johnson	&	U	&	12.56	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	699	&	Johnson	&	U	&	12.57	&	0.05	&	\citet{1954ApJ...120..196J}\\
GJ	699	&	Johnson	&	U	&	12.57	&	0.05	&	\citet{1955AnAp...18..292J}\\
GJ	699	&	Johnson	&	U	&	12.57	&	0.05	&	\citet{1965S_T....30...21I}\\
GJ	699	&	Johnson	&	U	&	12.57	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	699	&	Johnson	&	U	&	12.57	&	0.05	&	\citet{1964BOTT....3..305J}\\
GJ	699	&	Johnson	&	B	&	11.28	&	0.05	&	\citet{1978A_AS...34....1N}\\
GJ	699	&	Johnson	&	B	&	11.29	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	699	&	Johnson	&	B	&	11.29	&	0.05	&	\citet{1976ApJ...208..776H}\\
GJ	699	&	Johnson	&	B	&	11.29	&	0.05	&	\citet{1984SAAOC...8...59C}\\
GJ	699	&	Johnson	&	B	&	11.27	&	0.05	&	\citet{1982MNRAS.201...51R}\\
GJ	699	&	Johnson	&	B	&	11.29	&	0.05	&	\citet{1983AJ.....88..439L}\\
GJ	699	&	Johnson	&	B	&	11.26	&	0.05	&	\citet{1973PASP...85..721U}\\
GJ	699	&	Johnson	&	B	&	11.28	&	0.05	&	\citet{1976PUSNO..24c...1D}\\
GJ	699	&	Johnson	&	B	&	11.27	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	699	&	Johnson	&	B	&	11.28	&	0.05	&	\citet{1954ApJ...120..196J}\\
GJ	699	&	Johnson	&	B	&	11.28	&	0.05	&	\citet{1955AnAp...18..292J}\\
GJ	699	&	Johnson	&	B	&	11.28	&	0.05	&	\citet{1965S_T....30...21I}\\
GJ	699	&	Johnson	&	B	&	11.28	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	699	&	Johnson	&	B	&	11.28	&	0.05	&	\citet{1964BOTT....3..305J}\\
GJ	699	&	Johnson	&	V	&	9.54	&	0.05	&	\citet{1978A_AS...34....1N}\\
GJ	699	&	Johnson	&	V	&	9.54	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	699	&	Johnson	&	V	&	9.54	&	0.05	&	\citet{1976ApJ...208..776H}\\
GJ	699	&	Johnson	&	V	&	9.56	&	0.05	&	\citet{1984SAAOC...8...59C}\\
GJ	699	&	Johnson	&	V	&	9.57	&	0.05	&	\citet{1982MNRAS.201...51R}\\
GJ	699	&	Johnson	&	V	&	9.55	&	0.05	&	\citet{1983AJ.....88..439L}\\
GJ	699	&	Johnson	&	V	&	9.52	&	0.05	&	\citet{1973PASP...85..721U}\\
GJ	699	&	Johnson	&	V	&	9.54	&	0.05	&	\citet{1976PUSNO..24c...1D}\\
GJ	699	&	Johnson	&	V	&	9.53	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	699	&	Johnson	&	V	&	9.54	&	0.05	&	\citet{1954ApJ...120..196J}\\
GJ	699	&	Johnson	&	V	&	9.54	&	0.05	&	\citet{1955AnAp...18..292J}\\
GJ	699	&	Johnson	&	V	&	9.54	&	0.05	&	\citet{1965S_T....30...21I}\\
GJ	699	&	Johnson	&	V	&	9.54	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	699	&	Johnson	&	V	&	9.54	&	0.05	&	\citet{1964BOTT....3..305J}\\
GJ	699	&	Johnson	&	R	&	7.71	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	699	&	Johnson	&	R	&	7.71	&	0.05	&	\citet{1964BOTT....3..305J}\\
GJ	699	&	Johnson	&	I	&	6.03	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	699	&	Johnson	&	I	&	6.1	&	0.05	&	\citet{1964BOTT....3..305J}\\
GJ	699	&	1000	&	200	&	6.39	&	0.05	&	\citet{1978ApJ...220..935M}\\
GJ	699	&	1250	&	250	&	5.45	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	699	&	1250	&	250	&	5.27	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	699	&	1250	&	250	&	5.3	&	0.05	&	\citet{1976ApJ...208..399M}\\
GJ	699	&	1250	&	250	&	5.28	&	0.05	&	\citet{1977AJ.....82..729P}\\
GJ	699	&	1250	&	250	&	5.41	&	0.05	&	\citet{1984MNRAS.206...19R}\\
GJ	699	&	1250	&	250	&	5.33	&	0.05	&	\citet{1986ApJS...61..531S}\\
GJ	699	&	1250	&	250	&	5.26	&	0.05	&	\citet{1990AJ....100..825C}\\
GJ	699	&	Johnson	&	J	&	5.45	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	699	&	Johnson	&	J	&	5.5	&	0.05	&	\citet{1964BOTT....3..305J}\\
GJ	699	&	Johnson	&	J	&	5.3	&	0.05	&	\citet{1976ApJ...208..399M}\\
GJ	699	&	Johnson	&	J	&	5.27	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	699	&	1290	&	258	&	5.28	&	0.05	&	\citet{1993AJ....105.1045T}\\
GJ	699	&	1630	&	326	&	4.79	&	0.05	&	\citet{1990AJ....100..825C}\\
GJ	699	&	1650	&	330	&	4.78	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	699	&	1650	&	330	&	4.75	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	699	&	1650	&	330	&	4.77	&	0.05	&	\citet{1976ApJ...208..399M}\\
GJ	699	&	1650	&	330	&	4.76	&	0.05	&	\citet{1977AJ.....82..729P}\\
GJ	699	&	1650	&	330	&	4.83	&	0.05	&	\citet{1984MNRAS.206...19R}\\
GJ	699	&	1650	&	330	&	4.82	&	0.05	&	\citet{1986ApJS...61..531S}\\
GJ	699	&	Johnson	&	H	&	4.77	&	0.05	&	\citet{1976ApJ...208..399M}\\
GJ	699	&	Johnson	&	H	&	4.75	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	699	&	Johnson	&	H	&	4.78	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	699	&	1670	&	334	&	4.77	&	0.05	&	\citet{1993AJ....105.1045T}\\
GJ	699	&	2200	&	440	&	4.53	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	699	&	2200	&	440	&	4.54	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	699	&	2200	&	440	&	4.5	&	0.05	&	\citet{1976ApJ...208..399M}\\
GJ	699	&	2200	&	440	&	4.56	&	0.05	&	\citet{1984MNRAS.206...19R}\\
GJ	699	&	2200	&	440	&	4.56	&	0.05	&	\citet{1986ApJS...61..531S}\\
GJ	699	&	2200	&	440	&	4.51	&	0.05	&	\citet{1990AJ....100..825C}\\
GJ	699	&	2200	&	440	&	4.49	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	699	&	2200	&	440	&	4.51	&	0.05	&	\citet{1977AJ.....82..729P}\\
GJ	699	&	Johnson	&	K	&	4.53	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	699	&	Johnson	&	K	&	4.64	&	0.05	&	\citet{1964BOTT....3..305J}\\
GJ	699	&	Johnson	&	K	&	4.5	&	0.05	&	\citet{1976ApJ...208..399M}\\
GJ	699	&	Johnson	&	K	&	4.49	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	699	&	Johnson	&	K	&	4.54	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	699	&	2230	&	446	&	4.52	&	0.05	&	\citet{1993AJ....105.1045T}\\
GJ	699	&	3400	&	680	&	4.17	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	699	&	3400	&	680	&	4.23	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	699	&	3500	&	700	&	4.2	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	699	&	3500	&	700	&	4.18	&	0.05	&	\citet{1976ApJ...208..399M}\\
GJ	699	&	Johnson	&	L	&	4.17	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	699	&	Johnson	&	L	&	4.18	&	0.05	&	\citet{1976ApJ...208..399M}\\
GJ	699	&	Johnson	&	L	&	4.23	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	699	&	Johnson	&	L	&	4.2	&	0.05	&	\citet{1974AJ.....79.1056V}\\
											
GJ	702A	&	Johnson	&	U	&	5.31	&	0.05	&	\citet{1965AJ.....70...19E}\\
GJ	702A	&	Johnson	&	U	&	5.6	&	0.05	&	\citet{1971PASP...83..488L}\\
GJ	702A	&	Johnson	&	B	&	4.98	&	0.05	&	\citet{1965AJ.....70...19E}\\
GJ	702A	&	Johnson	&	B	&	5.03	&	0.05	&	\citet{1971PASP...83..488L}\\
GJ	702A	&	Johnson	&	B	&	7.15	&	0.05	&	\citet{1965AJ.....70...19E}\\
GJ	702A	&	Johnson	&	V	&	4.2	&	0.05	&	\citet{1965AJ.....70...19E}\\
GJ	702A	&	Johnson	&	V	&	4.25	&	0.05	&	\citet{1971PASP...83..488L}\\
GJ	702A	&	Johnson	&	V	&	6	&	0.05	&	\citet{1965AJ.....70...19E}\\
GJ	702A	&	1240	&	248	&	2.41	&	0.05	&	\citet{1993AJ....106..773H}\\
GJ	702A	&	1250	&	250	&	2.49	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	702A	&	1250	&	250	&	2.49	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	702A	&	2Mass	&	J	&	2.34	&	0.3	&	\citet{2003tmc..book.....C}\\
GJ	702A	&	1280	&	256	&	2.4	&	0.05	&	\citet{1994A_AS..107..365A}\\
GJ	702A	&	1650	&	330	&	2.04	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	702A	&	1650	&	330	&	1.96	&	0.05	&	\citet{1994A_AS..107..365A}\\
GJ	702A	&	2Mass	&	H	&	1.88	&	0.24	&	\citet{2003tmc..book.....C}\\
GJ	702A	&	2Mass	&	Ks	&	1.79	&	0.3	&	\citet{2003tmc..book.....C}\\
GJ	702A	&	2190	&	438	&	1.87	&	0.05	&	\citet{1994A_AS..107..365A}\\
GJ	702A	&	2190	&	438	&	1.96	&	0.05	&	\citet{1993AJ....106..773H}\\
GJ	702A	&	2200	&	440	&	1.96	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	702A	&	2200	&	440	&	1.88	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	702A	&	2200	&	440	&	1.88	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	702A	&	2200	&	440	&	1.9	&	0.05	&	\citet{1990A_A...230...87H}\\
GJ	702A	&	3500	&	700	&	1.8	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	725A	&	Geneva	&	U	&	12.28	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	725A	&	Johnson	&	U	&	11.55	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	725A	&	Johnson	&	U	&	11.43	&	0.05	&	\citet{1976PASP...88..444K}\\
GJ	725A	&	Johnson	&	U	&	11.55	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	725A	&	Johnson	&	U	&	11.56	&	0.05	&	\citet{1978A_AS...34....1N}\\
GJ	725A	&	Geneva	&	B1	&	11.25	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	725A	&	Geneva	&	B	&	9.89	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	725A	&	Geneva	&	B2	&	10.96	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	725A	&	Johnson	&	B	&	10.44	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	725A	&	Johnson	&	B	&	10.43	&	0.05	&	\citet{1976PASP...88..444K}\\
GJ	725A	&	Johnson	&	B	&	10.52	&	0.05	&	\citet{1956AJ.....61..213M}\\
GJ	725A	&	Johnson	&	B	&	10.44	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	725A	&	Johnson	&	B	&	10.45	&	0.05	&	\citet{1978A_AS...34....1N}\\
GJ	725A	&	Geneva	&	V1	&	9.75	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	725A	&	Geneva	&	V	&	8.94	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	725A	&	Johnson	&	V	&	8.9	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	725A	&	Johnson	&	V	&	8.93	&	0.05	&	\citet{1976PASP...88..444K}\\
GJ	725A	&	Johnson	&	V	&	8.99	&	0.05	&	\citet{1956AJ.....61..213M}\\
GJ	725A	&	Johnson	&	V	&	8.9	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	725A	&	Johnson	&	V	&	8.91	&	0.05	&	\citet{1978A_AS...34....1N}\\
GJ	725A	&	Geneva	&	G	&	9.85	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	725A	&	Cousins	&	Rc	&	7.82	&	0.05	&	\citet{1995yCat.5070....0G}\\
GJ	725A	&	Cousins	&	Ic	&	6.48	&	0.05	&	\citet{1995yCat.5070....0G}\\
GJ	725A	&	2Mass	&	J	&	5.19	&	0	&	\citet{2003tmc..book.....C}\\
GJ	725A	&	2Mass	&	H	&	4.74	&	0.03	&	\citet{2003tmc..book.....C}\\
GJ	725A	&	Johnson	&	H	&	4.68	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	725A	&	2Mass	&	Ks	&	4.43	&	0.01	&	\citet{2003tmc..book.....C}\\
GJ	725A	&	Johnson	&	K	&	4.46	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	725A	&	Johnson	&	L	&	4.2	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	725B	&	Geneva	&	U	&	13.12	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	725B	&	Johnson	&	U	&	12.33	&	0.05	&	\citet{1983IBVS.2318....1W}\\
GJ	725B	&	Johnson	&	U	&	12.42	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	725B	&	Johnson	&	U	&	12.42	&	0.05	&	\citet{1978A_AS...34....1N}\\
GJ	725B	&	Johnson	&	U	&	12.42	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	725B	&	Geneva	&	B1	&	12.1	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	725B	&	Geneva	&	B	&	10.73	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	725B	&	Geneva	&	B2	&	11.78	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	725B	&	Johnson	&	B	&	11.24	&	0.05	&	\citet{1983IBVS.2318....1W}\\
GJ	725B	&	Johnson	&	B	&	11.28	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	725B	&	Johnson	&	B	&	11.28	&	0.05	&	\citet{1978A_AS...34....1N}\\
GJ	725B	&	Johnson	&	B	&	11.28	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	725B	&	Geneva	&	V1	&	10.51	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	725B	&	Geneva	&	V	&	9.71	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	725B	&	Johnson	&	V	&	9.67	&	0.05	&	\citet{1983IBVS.2318....1W}\\
GJ	725B	&	Johnson	&	V	&	9.69	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	725B	&	Johnson	&	V	&	9.69	&	0.05	&	\citet{1978A_AS...34....1N}\\
GJ	725B	&	Johnson	&	V	&	9.69	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	725B	&	Geneva	&	G	&	10.64	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	725B	&	Cousins	&	Rc	&	8.56	&	0.05	&	\citet{1995yCat.5070....0G}\\
GJ	725B	&	Cousins	&	Ic	&	7.13	&	0.05	&	\citet{1995yCat.5070....0G}\\
GJ	725B	&	2Mass	&	J	&	5.72	&	0.01	&	\citet{2003tmc..book.....C}\\
GJ	725B	&	2Mass	&	H	&	5.2	&	0.02	&	\citet{2003tmc..book.....C}\\
GJ	725B	&	Johnson	&	H	&	5.24	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	725B	&	2Mass	&	Ks	&	5	&	0.02	&	\citet{2003tmc..book.....C}\\
GJ	725B	&	Johnson	&	K	&	4.98	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	725B	&	Johnson	&	L	&	4.7	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	764	&	Geneva	&	U	&	6.27	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	764	&	Stromgren	&	u	&	7.02	&	0.08	&	\citet{1970AJ.....75..978C}\\
GJ	764	&	Stromgren	&	u	&	7.02	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	764	&	Stromgren	&	u	&	7.03	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	764	&	Stromgren	&	u	&	7.03	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	764	&	Stromgren	&	u	&	7.04	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	764	&	Johnson	&	U	&	5.82	&	0.05	&	\citet{1975MNRAS.172..667J}\\
GJ	764	&	Johnson	&	U	&	5.84	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	764	&	Johnson	&	U	&	5.84	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	764	&	Johnson	&	U	&	5.85	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	764	&	Johnson	&	U	&	5.85	&	0.05	&	\citet{1985A_AS...59..461O}\\
GJ	764	&	Johnson	&	U	&	5.85	&	0.05	&	\citet{1985A_AS...61..331O}\\
GJ	764	&	Johnson	&	U	&	5.85	&	0.05	&	\citet{1986A_AS...65..405O}\\
GJ	764	&	Johnson	&	U	&	5.86	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	764	&	Johnson	&	U	&	5.86	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	764	&	Johnson	&	U	&	5.86	&	0.05	&	\citet{1964BOTT....3..305J}\\
GJ	764	&	Johnson	&	U	&	5.86	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	764	&	Johnson	&	U	&	5.86	&	0.05	&	\citet{1971PASP...83...79F}\\
GJ	764	&	Johnson	&	U	&	5.86	&	0.05	&	\citet{1984A_AS...57..357O}\\
GJ	764	&	Johnson	&	U	&	5.87	&	0.05	&	\citet{1985A_AS...61..331O}\\
GJ	764	&	Johnson	&	U	&	5.87	&	0.05	&	\citet{1983A_AS...52..131O}\\
GJ	764	&	Geneva	&	B1	&	5.9	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	764	&	Stromgren	&	v	&	5.95	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	764	&	Stromgren	&	v	&	5.96	&	0.08	&	\citet{1970AJ.....75..978C}\\
GJ	764	&	Stromgren	&	v	&	5.97	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	764	&	Stromgren	&	v	&	5.97	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	764	&	Stromgren	&	v	&	5.97	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	764	&	Geneva	&	B	&	4.71	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	764	&	Johnson	&	B	&	5.44	&	0.05	&	\citet{1966ArA.....4..137H}\\
GJ	764	&	Johnson	&	B	&	5.45	&	0.05	&	\citet{1970Priv.........0H}\\
GJ	764	&	Johnson	&	B	&	5.46	&	0.05	&	\citet{1985A_AS...59..461O}\\
GJ	764	&	Johnson	&	B	&	5.46	&	0.05	&	\citet{1969ArA.....5..303H}\\
GJ	764	&	Johnson	&	B	&	5.46	&	0.05	&	\citet{1985A_AS...61..331O}\\
GJ	764	&	Johnson	&	B	&	5.46	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	764	&	Johnson	&	B	&	5.46	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	764	&	Johnson	&	B	&	5.46	&	0.05	&	\citet{1984A_AS...57..357O}\\
GJ	764	&	Johnson	&	B	&	5.47	&	0.05	&	\citet{1986A_AS...65..405O}\\
GJ	764	&	Johnson	&	B	&	5.47	&	0.05	&	\citet{1983A_AS...52..131O}\\
GJ	764	&	Johnson	&	B	&	5.47	&	0.05	&	\citet{1985A_AS...61..331O}\\
GJ	764	&	Johnson	&	B	&	5.47	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	764	&	Johnson	&	B	&	5.47	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	764	&	Johnson	&	B	&	5.47	&	0.05	&	\citet{1971PASP...83...79F}\\
GJ	764	&	Johnson	&	B	&	5.48	&	0.05	&	\citet{1975MNRAS.172..667J}\\
GJ	764	&	Johnson	&	B	&	5.49	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	764	&	Johnson	&	B	&	5.49	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	764	&	Johnson	&	B	&	5.49	&	0.05	&	\citet{1964BOTT....3..305J}\\
GJ	764	&	Johnson	&	B	&	5.49	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	764	&	Johnson	&	B	&	5.5	&	0.05	&	\citet{1963ArA.....3..273O}\\
GJ	764	&	Johnson	&	B	&	5.54	&	0.05	&	\citet{1979PASP...91..180M}\\
GJ	764	&	Geneva	&	B2	&	5.94	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	764	&	Stromgren	&	b	&	5.17	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	764	&	Stromgren	&	b	&	5.17	&	0.08	&	\citet{1970AJ.....75..978C}\\
GJ	764	&	Stromgren	&	b	&	5.17	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	764	&	Stromgren	&	b	&	5.17	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	764	&	Stromgren	&	b	&	5.18	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	764	&	Stromgren	&	b	&	5.18	&	0.08	&	\citet{1992PASP..104..911T}\\
GJ	764	&	Geneva	&	V1	&	5.45	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	764	&	Stromgren	&	y	&	4.7	&	0.08	&	\citet{1970AJ.....75..978C}\\
GJ	764	&	Stromgren	&	y	&	4.7	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	764	&	Stromgren	&	y	&	4.7	&	0.08	&	\citet{1992PASP..104..911T}\\
GJ	764	&	Stromgren	&	y	&	4.7	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	764	&	Stromgren	&	y	&	4.7	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	764	&	Geneva	&	V	&	4.67	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	764	&	Johnson	&	V	&	4.67	&	0.05	&	\citet{1985A_AS...59..461O}\\
GJ	764	&	Johnson	&	V	&	4.67	&	0.05	&	\citet{1966ArA.....4..137H}\\
GJ	764	&	Johnson	&	V	&	4.67	&	0.05	&	\citet{1969ArA.....5..303H}\\
GJ	764	&	Johnson	&	V	&	4.67	&	0.05	&	\citet{1983A_AS...52..131O}\\
GJ	764	&	Johnson	&	V	&	4.67	&	0.05	&	\citet{1984A_AS...57..357O}\\
GJ	764	&	Johnson	&	V	&	4.67	&	0.05	&	\citet{1986A_AS...65..405O}\\
GJ	764	&	Johnson	&	V	&	4.68	&	0.05	&	\citet{1970Priv.........0H}\\
GJ	764	&	Johnson	&	V	&	4.68	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	764	&	Johnson	&	V	&	4.68	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	764	&	Johnson	&	V	&	4.68	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	764	&	Johnson	&	V	&	4.68	&	0.05	&	\citet{1971PASP...83...79F}\\
GJ	764	&	Johnson	&	V	&	4.68	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	764	&	Johnson	&	V	&	4.68	&	0.05	&	\citet{1985A_AS...61..331O}\\
GJ	764	&	Johnson	&	V	&	4.69	&	0.05	&	\citet{1975MNRAS.172..667J}\\
GJ	764	&	Johnson	&	V	&	4.69	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	764	&	Johnson	&	V	&	4.69	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	764	&	Johnson	&	V	&	4.69	&	0.05	&	\citet{1964BOTT....3..305J}\\
GJ	764	&	Johnson	&	V	&	4.69	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	764	&	Johnson	&	V	&	4.69	&	0.05	&	\citet{1985A_AS...61..331O}\\
GJ	764	&	Johnson	&	V	&	4.71	&	0.05	&	\citet{1963ArA.....3..273O}\\
GJ	764	&	Johnson	&	V	&	4.75	&	0.05	&	\citet{1979PASP...91..180M}\\
GJ	764	&	Geneva	&	G	&	5.67	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	764	&	Johnson	&	R	&	4.04	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	764	&	Johnson	&	I	&	3.63	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	764	&	1250	&	250	&	3.32	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	764	&	1250	&	250	&	3.32	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	764	&	1250	&	250	&	3.34	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	764	&	2200	&	440	&	2.78	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	764	&	2200	&	440	&	2.78	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	764	&	2200	&	440	&	2.86	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	764	&	3400	&	680	&	2.53	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	764	&	3400	&	680	&	2.63	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	809	&	Geneva	&	U	&	11.85	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	809	&	Johnson	&	U	&	11.23	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	809	&	Johnson	&	U	&	11.24	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	809	&	Johnson	&	U	&	11.25	&	0.05	&	\citet{1971BOTT....6..143I}\\
GJ	809	&	Geneva	&	B1	&	10.87	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	809	&	Geneva	&	B	&	9.44	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	809	&	Geneva	&	B2	&	10.45	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	809	&	Johnson	&	B	&	9.99	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	809	&	Johnson	&	B	&	10.06	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	809	&	Johnson	&	B	&	10	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	809	&	Johnson	&	B	&	10.04	&	0.05	&	\citet{1971BOTT....6..143I}\\
GJ	809	&	Geneva	&	V1	&	9.38	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	809	&	Geneva	&	V	&	8.55	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	809	&	Johnson	&	V	&	8.5	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	809	&	Johnson	&	V	&	8.58	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	809	&	Johnson	&	V	&	8.5	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	809	&	Johnson	&	V	&	8.58	&	0.05	&	\citet{1971BOTT....6..143I}\\
GJ	809	&	Geneva	&	G	&	9.38	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	809	&	Cousins	&	Rc	&	7.61	&	0.05	&	\citet{1995yCat.5070....0G}\\
GJ	809	&	Cousins	&	Ic	&	6.58	&	0.05	&	\citet{1995yCat.5070....0G}\\
GJ	809	&	1250	&	250	&	5.52	&	0.05	&	\citet{1977AJ.....82..729P}\\
GJ	809	&	2Mass	&	J	&	5.43	&	0.02	&	\citet{2003tmc..book.....C}\\
GJ	809	&	1650	&	330	&	4.8	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	809	&	1650	&	330	&	4.81	&	0.05	&	\citet{1977AJ.....82..729P}\\
GJ	809	&	1650	&	330	&	11.13	&	0.05	&	\citet{1996AJ....112.2238S}\\
GJ	809	&	2Mass	&	H	&	4.92	&	0.06	&	\citet{2003tmc..book.....C}\\
GJ	809	&	Johnson	&	H	&	4.8	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	809	&	2100	&	420	&	10.28	&	0.05	&	\citet{1996AJ....112.2238S}\\
GJ	809	&	2Mass	&	Ks	&	4.62	&	0.02	&	\citet{2003tmc..book.....C}\\
GJ	809	&	2200	&	440	&	4.62	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	809	&	2200	&	440	&	4.64	&	0.05	&	\citet{1977AJ.....82..729P}\\
GJ	809	&	Johnson	&	K	&	4.62	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	809	&	3500	&	700	&	4.4	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	809	&	Johnson	&	L	&	4.4	&	0.05	&	\citet{1974AJ.....79.1056V}\\
											
GJ	820A	&	Johnson	&	U	&	7.48	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	820A	&	Johnson	&	U	&	7.48	&	0.05	&	\citet{1953ApJ...117..361J}\\
GJ	820A	&	Johnson	&	U	&	7.48	&	0.05	&	\citet{1955AnAp...18..292J}\\
GJ	820A	&	Johnson	&	U	&	7.48	&	0.05	&	\citet{1971PASP...83..488L}\\
GJ	820A	&	Johnson	&	U	&	7.48	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	820A	&	Johnson	&	U	&	7.5	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	820A	&	Johnson	&	U	&	7.5	&	0.05	&	\citet{1963AJ.....68..483E}\\
GJ	820A	&	Johnson	&	U	&	7.5	&	0.05	&	\citet{1964AJ.....69..215M}\\
GJ	820A	&	Johnson	&	U	&	7.5	&	0.05	&	\citet{1964BOTT....3..305J}\\
GJ	820A	&	Johnson	&	U	&	7.5	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	820A	&	Johnson	&	U	&	7.5	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	820A	&	Johnson	&	U	&	7.5	&	0.05	&	\citet{1978A_AS...34....1N}\\
GJ	820A	&	Johnson	&	U	&	7.51	&	0.05	&	\citet{1971A_A....12..442M}\\
GJ	820A	&	Johnson	&	U	&	7.51	&	0.05	&	\citet{1963MNRAS.125..557A}\\
GJ	820A	&	Johnson	&	U	&	7.52	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	820A	&	Johnson	&	U	&	7.53	&	0.05	&	\citet{1975MNRAS.172..667J}\\
GJ	820A	&	Johnson	&	U	&	7.53	&	0.05	&	\citet{1965S_T....30...21I}\\
GJ	820A	&	Johnson	&	U	&	7.56	&	0.05	&	\citet{1979A_AS...36..297B}\\
GJ	820A	&	Johnson	&	U	&	7.57	&	0.05	&	\citet{1964ApJ...139.1105T}\\
GJ	820A	&	Johnson	&	B	&	6.38	&	0.05	&	\citet{1971A_A....12..442M}\\
GJ	820A	&	Johnson	&	B	&	6.38	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	820A	&	Johnson	&	B	&	6.38	&	0.05	&	\citet{1953ApJ...117..361J}\\
GJ	820A	&	Johnson	&	B	&	6.38	&	0.05	&	\citet{1955AnAp...18..292J}\\
GJ	820A	&	Johnson	&	B	&	6.38	&	0.05	&	\citet{1971PASP...83..488L}\\
GJ	820A	&	Johnson	&	B	&	6.38	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	820A	&	Johnson	&	B	&	6.39	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	820A	&	Johnson	&	B	&	6.39	&	0.05	&	\citet{1964AJ.....69..215M}\\
GJ	820A	&	Johnson	&	B	&	6.39	&	0.05	&	\citet{1964BOTT....3..305J}\\
GJ	820A	&	Johnson	&	B	&	6.39	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	820A	&	Johnson	&	B	&	6.39	&	0.05	&	\citet{1978A_AS...34....1N}\\
GJ	820A	&	Johnson	&	B	&	6.4	&	0.05	&	\citet{1963AJ.....68..483E}\\
GJ	820A	&	Johnson	&	B	&	6.4	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	820A	&	Johnson	&	B	&	6.4	&	0.05	&	\citet{1979A_AS...36..297B}\\
GJ	820A	&	Johnson	&	B	&	6.4	&	0.05	&	\citet{1979PASP...91..180M}\\
GJ	820A	&	Johnson	&	B	&	6.41	&	0.05	&	\citet{1974A_AS...18..169N}\\
GJ	820A	&	Johnson	&	B	&	6.41	&	0.05	&	\citet{1963MNRAS.125..557A}\\
GJ	820A	&	Johnson	&	B	&	6.42	&	0.05	&	\citet{1975MNRAS.172..667J}\\
GJ	820A	&	Johnson	&	B	&	6.42	&	0.05	&	\citet{1965S_T....30...21I}\\
GJ	820A	&	Johnson	&	B	&	6.43	&	0.05	&	\citet{1964ApJ...139.1105T}\\
GJ	820A	&	Johnson	&	B	&	6.43	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	820A	&	Johnson	&	V	&	5.19	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	820A	&	Johnson	&	V	&	5.19	&	0.05	&	\citet{1953ApJ...117..361J}\\
GJ	820A	&	Johnson	&	V	&	5.19	&	0.05	&	\citet{1955AnAp...18..292J}\\
GJ	820A	&	Johnson	&	V	&	5.19	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	820A	&	Johnson	&	V	&	5.2	&	0.05	&	\citet{1971PASP...83..488L}\\
GJ	820A	&	Johnson	&	V	&	5.21	&	0.05	&	\citet{1978A_AS...34....1N}\\
GJ	820A	&	Johnson	&	V	&	5.22	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	820A	&	Johnson	&	V	&	5.22	&	0.05	&	\citet{1963AJ.....68..483E}\\
GJ	820A	&	Johnson	&	V	&	5.22	&	0.05	&	\citet{1964ApJ...139.1105T}\\
GJ	820A	&	Johnson	&	V	&	5.22	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	820A	&	Johnson	&	V	&	5.23	&	0.05	&	\citet{1964BOTT....3..305J}\\
GJ	820A	&	Johnson	&	V	&	5.23	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	820A	&	Johnson	&	V	&	5.24	&	0.05	&	\citet{1975MNRAS.172..667J}\\
GJ	820A	&	Johnson	&	V	&	5.24	&	0.05	&	\citet{1971A_A....12..442M}\\
GJ	820A	&	Johnson	&	V	&	5.24	&	0.05	&	\citet{1963MNRAS.125..557A}\\
GJ	820A	&	Johnson	&	V	&	5.24	&	0.05	&	\citet{1974A_AS...18..169N}\\
GJ	820A	&	Johnson	&	V	&	5.25	&	0.05	&	\citet{1965S_T....30...21I}\\
GJ	820A	&	Johnson	&	V	&	5.26	&	0.05	&	\citet{1979PASP...91..180M}\\
GJ	820A	&	Johnson	&	V	&	5.26	&	0.05	&	\citet{1979A_AS...36..297B}\\
GJ	820A	&	Johnson	&	V	&	5.27	&	0.05	&	\citet{1964AJ.....69..215M}\\
GJ	820A	&	Johnson	&	V	&	5.27	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	820A	&	Johnson	&	R	&	4.19	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	820A	&	Johnson	&	R	&	4.25	&	0.05	&	\citet{1971A_A....12..442M}\\
GJ	820A	&	Johnson	&	I	&	3.39	&	0.1	&	\citet{1969tmss.book.....N}\\
GJ	820A	&	Johnson	&	I	&	3.54	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	820A	&	Johnson	&	J	&	3.15	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	820A	&	Johnson	&	J	&	3.16	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	820A	&	Johnson	&	H	&	2.47	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	820A	&	Johnson	&	H	&	2.61	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	820A	&	Johnson	&	K	&	1.71	&	0.04	&	\citet{1969tmss.book.....N}\\
GJ	820A	&	Johnson	&	K	&	2.37	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	820A	&	Johnson	&	K	&	2.39	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	820A	&	Johnson	&	K	&	2.4	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	820A	&	Johnson	&	L	&	2.3	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	820A	&	Johnson	&	L	&	2.31	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	820A	&	Johnson	&	L	&	2.31	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	820B	&	Stromgren	&	u	&	9.82	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	820B	&	Stromgren	&	u	&	9.82	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	820B	&	Stromgren	&	u	&	9.82	&	0.08	&	\citet{1970ApJS...22..117B}\\
GJ	820B	&	Stromgren	&	u	&	9.82	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	820B	&	Stromgren	&	u	&	9.82	&	0.08	&	\citet{1970AJ.....75..978C}\\
GJ	820B	&	Stromgren	&	u	&	9.83	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	820B	&	Johnson	&	U	&	8.61	&	0.05	&	\citet{1971PASP...83..488L}\\
GJ	820B	&	Johnson	&	U	&	8.62	&	0.05	&	\citet{1971A_A....12..442M}\\
GJ	820B	&	Johnson	&	U	&	8.62	&	0.05	&	\citet{1964BOTT....3..305J}\\
GJ	820B	&	Johnson	&	U	&	8.62	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	820B	&	Johnson	&	U	&	8.62	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	820B	&	Johnson	&	U	&	8.63	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	820B	&	Johnson	&	U	&	8.63	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	820B	&	Johnson	&	U	&	8.63	&	0.05	&	\citet{1953ApJ...117..361J}\\
GJ	820B	&	Johnson	&	U	&	8.63	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	820B	&	Johnson	&	U	&	8.65	&	0.05	&	\citet{1963MNRAS.125..557A}\\
GJ	820B	&	Johnson	&	U	&	8.65	&	0.05	&	\citet{1975MNRAS.172..667J}\\
GJ	820B	&	Johnson	&	U	&	8.65	&	0.05	&	\citet{1979A_AS...36..297B}\\
GJ	820B	&	Johnson	&	U	&	8.66	&	0.05	&	\citet{1964ApJ...139.1105T}\\
GJ	820B	&	Johnson	&	U	&	8.66	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	820B	&	Stromgren	&	v	&	8.25	&	0.08	&	\citet{1970ApJS...22..117B}\\
GJ	820B	&	Stromgren	&	v	&	8.28	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	820B	&	Stromgren	&	v	&	8.29	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	820B	&	Stromgren	&	v	&	8.29	&	0.08	&	\citet{1970AJ.....75..978C}\\
GJ	820B	&	Stromgren	&	v	&	8.29	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	820B	&	Stromgren	&	v	&	8.29	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	820B	&	Johnson	&	B	&	7.38	&	0.05	&	\citet{1964BOTT....3..305J}\\
GJ	820B	&	Johnson	&	B	&	7.38	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	820B	&	Johnson	&	B	&	7.39	&	0.05	&	\citet{1971A_A....12..442M}\\
GJ	820B	&	Johnson	&	B	&	7.4	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	820B	&	Johnson	&	B	&	7.4	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	820B	&	Johnson	&	B	&	7.4	&	0.05	&	\citet{1953ApJ...117..361J}\\
GJ	820B	&	Johnson	&	B	&	7.4	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	820B	&	Johnson	&	B	&	7.4	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	820B	&	Johnson	&	B	&	7.4	&	0.05	&	\citet{1971PASP...83..488L}\\
GJ	820B	&	Johnson	&	B	&	7.41	&	0.05	&	\citet{1979PASP...91..180M}\\
GJ	820B	&	Johnson	&	B	&	7.41	&	0.05	&	\citet{1979A_AS...36..297B}\\
GJ	820B	&	Johnson	&	B	&	7.42	&	0.05	&	\citet{1963MNRAS.125..557A}\\
GJ	820B	&	Johnson	&	B	&	7.42	&	0.05	&	\citet{1964ApJ...139.1105T}\\
GJ	820B	&	Johnson	&	B	&	7.43	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	820B	&	Johnson	&	B	&	7.43	&	0.05	&	\citet{1975MNRAS.172..667J}\\
GJ	820B	&	Stromgren	&	b	&	6.82	&	0.08	&	\citet{1970AJ.....75..978C}\\
GJ	820B	&	Stromgren	&	b	&	6.82	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	820B	&	Stromgren	&	b	&	6.82	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	820B	&	Stromgren	&	b	&	6.82	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	820B	&	Stromgren	&	b	&	6.83	&	0.08	&	\citet{1970ApJS...22..117B}\\
GJ	820B	&	Stromgren	&	y	&	6.03	&	0.08	&	\citet{1970AJ.....75..978C}\\
GJ	820B	&	Stromgren	&	y	&	6.03	&	0.08	&	\citet{1970ApJS...22..117B}\\
GJ	820B	&	Stromgren	&	y	&	6.03	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	820B	&	Stromgren	&	y	&	6.03	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	820B	&	Stromgren	&	y	&	6.03	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	820B	&	Johnson	&	V	&	6.02	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	820B	&	Johnson	&	V	&	6.02	&	0.05	&	\citet{1953ApJ...117..361J}\\
GJ	820B	&	Johnson	&	V	&	6.02	&	0.05	&	\citet{1964BOTT....3..305J}\\
GJ	820B	&	Johnson	&	V	&	6.02	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	820B	&	Johnson	&	V	&	6.02	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	820B	&	Johnson	&	V	&	6.03	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	820B	&	Johnson	&	V	&	6.03	&	0.05	&	\citet{1971PASP...83..488L}\\
GJ	820B	&	Johnson	&	V	&	6.04	&	0.05	&	\citet{1964ApJ...139.1105T}\\
GJ	820B	&	Johnson	&	V	&	6.05	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	820B	&	Johnson	&	V	&	6.06	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	820B	&	Johnson	&	V	&	6.06	&	0.05	&	\citet{1975MNRAS.172..667J}\\
GJ	820B	&	Johnson	&	V	&	6.07	&	0.05	&	\citet{1971A_A....12..442M}\\
GJ	820B	&	Johnson	&	V	&	6.07	&	0.05	&	\citet{1963MNRAS.125..557A}\\
GJ	820B	&	Johnson	&	V	&	6.09	&	0.05	&	\citet{1979PASP...91..180M}\\
GJ	820B	&	Johnson	&	V	&	6.09	&	0.05	&	\citet{1979A_AS...36..297B}\\
GJ	820B	&	Johnson	&	R	&	4.86	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	820B	&	Johnson	&	R	&	4.9	&	0.05	&	\citet{1971A_A....12..442M}\\
GJ	820B	&	Johnson	&	I	&	4.03	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	820B	&	Johnson	&	J	&	3.55	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	820B	&	Johnson	&	J	&	3.58	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	820B	&	Johnson	&	H	&	2.84	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	820B	&	Johnson	&	H	&	2.93	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	820B	&	Johnson	&	K	&	2.71	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	820B	&	Johnson	&	K	&	2.73	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	820B	&	Johnson	&	K	&	2.73	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	820B	&	Johnson	&	L	&	2.6	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	820B	&	Johnson	&	L	&	2.61	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	820B	&	Johnson	&	L	&	2.64	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	845	&	Geneva	&	U	&	7.14	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	845	&	Johnson	&	U	&	6.72	&	0.1	&	\citet{1962RGOB...64..103C}\\
GJ	845	&	Johnson	&	U	&	6.74	&	0.1	&	\citet{1966CoLPL...4...99J}\\
GJ	845	&	Johnson	&	U	&	6.75	&	0.1	&	\citet{1986EgUBV........0M}\\
GJ	845	&	Geneva	&	B1	&	6.46	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	845	&	Geneva	&	B	&	5.08	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	845	&	Johnson	&	B	&	5.72	&	0.1	&	\citet{1962RGOB...64..103C}\\
GJ	845	&	Johnson	&	B	&	5.73	&	0.1	&	\citet{1961ApJS....6..253I}\\
GJ	845	&	Johnson	&	B	&	5.74	&	0.1	&	\citet{1969BOTT....5...57M}\\
GJ	845	&	Johnson	&	B	&	5.75	&	0.1	&	\citet{1966CoLPL...4...99J}\\
GJ	845	&	Johnson	&	B	&	5.75	&	0.1	&	\citet{1986EgUBV........0M}\\
GJ	845	&	Johnson	&	B	&	5.76	&	0.1	&	\citet{1962RGOB...64..103C}\\
GJ	845	&	Geneva	&	B2	&	6.16	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	845	&	Geneva	&	V1	&	5.49	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	845	&	Geneva	&	V	&	4.69	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	845	&	Johnson	&	V	&	4.65	&	0.05	&	\citet{1961ApJS....6..253I}\\
GJ	845	&	Johnson	&	V	&	4.67	&	0.05	&	\citet{1962RGOB...64..103C}\\
GJ	845	&	Johnson	&	V	&	4.69	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	845	&	Johnson	&	V	&	4.69	&	0.05	&	\citet{1969BOTT....5...57M}\\
GJ	845	&	Johnson	&	V	&	4.69	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	845	&	Johnson	&	V	&	4.7	&	0.05	&	\citet{1962RGOB...64..103C}\\
GJ	845	&	Geneva	&	G	&	5.59	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	845	&	1250	&	250	&	2.83	&	0.05	&	\citet{1976ApJ...208..399M}\\
GJ	845	&	1650	&	330	&	2.3	&	0.05	&	\citet{1976ApJ...208..399M}\\
GJ	845	&	2200	&	440	&	2.18	&	0.05	&	\citet{1976ApJ...208..399M}\\
GJ	845	&	3500	&	700	&	2.12	&	0.05	&	\citet{1976ApJ...208..399M}\\
GJ	880	&	Johnson	&	U	&	11.34	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	880	&	Johnson	&	U	&	11.37	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	880	&	Johnson	&	U	&	11.4	&	0.05	&	\citet{1971BOTT....6..143I}\\
GJ	880	&	Johnson	&	B	&	10.17	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	880	&	Johnson	&	B	&	10.12	&	0.05	&	\citet{1956AJ.....61..213M}\\
GJ	880	&	Johnson	&	B	&	10.2	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	880	&	Johnson	&	B	&	10.19	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	880	&	Johnson	&	B	&	10.18	&	0.05	&	\citet{1971BOTT....6..143I}\\
GJ	880	&	Johnson	&	V	&	8.66	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	880	&	Johnson	&	V	&	8.6	&	0.05	&	\citet{1956AJ.....61..213M}\\
GJ	880	&	Johnson	&	V	&	8.68	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	880	&	Johnson	&	V	&	8.68	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	880	&	Johnson	&	V	&	8.68	&	0.05	&	\citet{1971BOTT....6..143I}\\
GJ	880	&	Johnson	&	R	&	7.24	&	0.05	&	\citet{1971BOTT....6..143I}\\
GJ	880	&	Johnson	&	I	&	6.1	&	0.05	&	\citet{1971BOTT....6..143I}\\
GJ	880	&	1250	&	250	&	5.38	&	0.05	&	\citet{1988MNRAS.234.1065L}\\
GJ	880	&	1250	&	250	&	5.33	&	0.05	&	\citet{1996AJ....112.2238S}\\
GJ	880	&	2Mass	&	J	&	5.36	&	0.01	&	\citet{2003tmc..book.....C}\\
GJ	880	&	Johnson	&	J	&	5.41	&	0.05	&	\citet{1971BOTT....6..143I}\\
GJ	880	&	1650	&	330	&	4.74	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	880	&	1650	&	330	&	4.75	&	0.05	&	\citet{1988MNRAS.234.1065L}\\
GJ	880	&	1650	&	330	&	4.7	&	0.05	&	\citet{1996AJ....112.2238S}\\
GJ	880	&	2Mass	&	H	&	4.8	&	0.03	&	\citet{2003tmc..book.....C}\\
GJ	880	&	Johnson	&	H	&	4.78	&	0.05	&	\citet{1971BOTT....6..143I}\\
GJ	880	&	Johnson	&	H	&	4.74	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	880	&	2100	&	420	&	4.52	&	0.05	&	\citet{1996AJ....112.2238S}\\
GJ	880	&	2Mass	&	Ks	&	4.52	&	0.01	&	\citet{2003tmc..book.....C}\\
GJ	880	&	2200	&	440	&	4.55	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	880	&	2200	&	440	&	4.53	&	0.05	&	\citet{1988MNRAS.234.1065L}\\
GJ	880	&	Johnson	&	K	&	4.58	&	0.05	&	\citet{1971BOTT....6..143I}\\
GJ	880	&	Johnson	&	K	&	4.55	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	880	&	3500	&	700	&	4.4	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	880	&	Johnson	&	L	&	4.38	&	0.05	&	\citet{1971BOTT....6..143I}\\
GJ	880	&	Johnson	&	L	&	4.4	&	0.05	&	\citet{1974AJ.....79.1056V}\\
GJ	887	&	Geneva	&	U	&	10.68	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	887	&	Johnson	&	U	&	10.02	&	0.1	&	\citet{1973MNSSA..32...11C}\\
GJ	887	&	Johnson	&	U	&	10.02	&	0.1	&	\citet{1986EgUBV........0M}\\
GJ	887	&	Geneva	&	B1	&	9.73	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	887	&	Geneva	&	B	&	8.28	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	887	&	Johnson	&	B	&	8.81	&	0.1	&	\citet{1962RGOB...64..103C}\\
GJ	887	&	Johnson	&	B	&	8.82	&	0.1	&	\citet{1963MNSSA..22..157S}\\
GJ	887	&	Johnson	&	B	&	8.84	&	0.1	&	\citet{1973MNSSA..32...11C}\\
GJ	887	&	Johnson	&	B	&	8.85	&	0.1	&	\citet{1986EgUBV........0M}\\
GJ	887	&	Geneva	&	B2	&	9.32	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	887	&	Geneva	&	V1	&	8.18	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	887	&	Geneva	&	V	&	7.35	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	887	&	Johnson	&	V	&	7.33	&	0.05	&	\citet{1962RGOB...64..103C}\\
GJ	887	&	Johnson	&	V	&	7.34	&	0.05	&	\citet{1973MNSSA..32...11C}\\
GJ	887	&	Johnson	&	V	&	7.36	&	0.05	&	\citet{1963MNSSA..22..157S}\\
GJ	887	&	Johnson	&	V	&	7.37	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	887	&	Geneva	&	G	&	8.17	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	887	&	1250	&	250	&	4.15	&	0.05	&	\citet{1988MNRAS.234.1065L}\\
GJ	887	&	1250	&	250	&	4.2	&	0.05	&	\citet{1976ApJ...208..399M}\\
GJ	887	&	1250	&	250	&	4.21	&	0.05	&	\citet{1994PASP..106..508M}\\
GJ	887	&	1650	&	330	&	3.59	&	0.05	&	\citet{1988MNRAS.234.1065L}\\
GJ	887	&	1650	&	330	&	3.6	&	0.05	&	\citet{1976ApJ...208..399M}\\
GJ	887	&	1650	&	330	&	3.6	&	0.05	&	\citet{1994PASP..106..508M}\\
GJ	887	&	2200	&	440	&	3.36	&	0.05	&	\citet{1976ApJ...208..399M}\\
GJ	887	&	2200	&	440	&	3.38	&	0.05	&	\citet{1994PASP..106..508M}\\
GJ	887	&	2200	&	440	&	3.38	&	0.05	&	\citet{1988MNRAS.234.1065L}\\
GJ	887	&	3500	&	700	&	3.2	&	0.05	&	\citet{1976ApJ...208..399M}\\
GJ	892	&	Geneva	&	U	&	7.9	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	892	&	Stromgren	&	u	&	8.66	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	892	&	Stromgren	&	u	&	8.65	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	892	&	Stromgren	&	u	&	8.68	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	892	&	Stromgren	&	u	&	8.71	&	0.08	&	\citet{1970ApJS...22..117B}\\
GJ	892	&	Stromgren	&	u	&	8.66	&	0.08	&	\citet{1990A_AS...82..531F}\\
GJ	892	&	Stromgren	&	u	&	8.66	&	0.08	&	\citet{1970AJ.....75..978C}\\
GJ	892	&	Stromgren	&	u	&	8.67	&	0.08	&	\citet{1973ApJ...179..855P}\\
GJ	892	&	Stromgren	&	u	&	8.7	&	0.08	&	\citet{1974AJ.....79.1424O}\\
GJ	892	&	Stromgren	&	u	&	8.58	&	0.08	&	\citet{1990AJ....100.1621P}\\
GJ	892	&	Johnson	&	U	&	7.46	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	892	&	Johnson	&	U	&	7.45	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	892	&	Johnson	&	U	&	7.43	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	892	&	Johnson	&	U	&	7.46	&	0.05	&	\citet{1966ZA.....64..269A}\\
GJ	892	&	Johnson	&	U	&	7.47	&	0.05	&	\citet{1983A_AS...52..131O}\\
GJ	892	&	Johnson	&	U	&	7.47	&	0.05	&	\citet{1954ApJ...120..196J}\\
GJ	892	&	Johnson	&	U	&	7.42	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	892	&	Johnson	&	U	&	7.45	&	0.05	&	\citet{1960BAN....15..199O}\\
GJ	892	&	Johnson	&	U	&	7.47	&	0.05	&	\citet{1984A_AS...57..357O}\\
GJ	892	&	Johnson	&	U	&	7.47	&	0.05	&	\citet{1985A_AS...59..461O}\\
GJ	892	&	Johnson	&	U	&	7.46	&	0.05	&	\citet{1986A_AS...65..405O}\\
GJ	892	&	Johnson	&	U	&	7.47	&	0.05	&	\citet{1964BOTT....3..305J}\\
GJ	892	&	Johnson	&	U	&	7.47	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	892	&	Johnson	&	U	&	7.45	&	0.05	&	\citet{1978AJ.....83..606M}\\
GJ	892	&	Johnson	&	U	&	7.45	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	892	&	Johnson	&	U	&	7.45	&	0.05	&	\citet{1975MNRAS.172..667J}\\
GJ	892	&	Johnson	&	U	&	7.48	&	0.05	&	\citet{1985A_AS...61..331O}\\
GJ	892	&	Johnson	&	U	&	7.46	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	892	&	Johnson	&	U	&	7.45	&	0.05	&	\citet{1974RMxAA...1...67M}\\
GJ	892	&	Johnson	&	U	&	7.44	&	0.05	&	\citet{1971A_A....12..442M}\\
GJ	892	&	Geneva	&	B1	&	7.22	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	892	&	Stromgren	&	v	&	7.27	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	892	&	Stromgren	&	v	&	7.25	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	892	&	Stromgren	&	v	&	7.28	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	892	&	Stromgren	&	v	&	7.27	&	0.08	&	\citet{1970ApJS...22..117B}\\
GJ	892	&	Stromgren	&	v	&	7.27	&	0.08	&	\citet{1990A_AS...82..531F}\\
GJ	892	&	Stromgren	&	v	&	7.27	&	0.08	&	\citet{1970AJ.....75..978C}\\
GJ	892	&	Stromgren	&	v	&	7.27	&	0.08	&	\citet{1973ApJ...179..855P}\\
GJ	892	&	Stromgren	&	v	&	7.26	&	0.08	&	\citet{1974AJ.....79.1424O}\\
GJ	892	&	Stromgren	&	v	&	7.24	&	0.08	&	\citet{1990AJ....100.1621P}\\
GJ	892	&	Geneva	&	B	&	5.86	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	892	&	Geneva	&	B2	&	6.99	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	892	&	Johnson	&	B	&	6.57	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	892	&	Johnson	&	B	&	6.55	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	892	&	Johnson	&	B	&	6.57	&	0.05	&	\citet{1966ZA.....64..269A}\\
GJ	892	&	Johnson	&	B	&	6.55	&	0.05	&	\citet{1983A_AS...52..131O}\\
GJ	892	&	Johnson	&	B	&	6.56	&	0.05	&	\citet{1952ApJ...116..251S}\\
GJ	892	&	Johnson	&	B	&	6.58	&	0.05	&	\citet{1954ApJ...120..196J}\\
GJ	892	&	Johnson	&	B	&	6.62	&	0.05	&	\citet{1963ArA.....3..273O}\\
GJ	892	&	Johnson	&	B	&	6.6	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	892	&	Johnson	&	B	&	6.55	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	892	&	Johnson	&	B	&	6.56	&	0.05	&	\citet{1960BAN....15..199O}\\
GJ	892	&	Johnson	&	B	&	6.55	&	0.05	&	\citet{1984A_AS...57..357O}\\
GJ	892	&	Johnson	&	B	&	6.56	&	0.05	&	\citet{1985A_AS...59..461O}\\
GJ	892	&	Johnson	&	B	&	6.56	&	0.05	&	\citet{1986A_AS...65..405O}\\
GJ	892	&	Johnson	&	B	&	6.58	&	0.05	&	\citet{1964BOTT....3..305J}\\
GJ	892	&	Johnson	&	B	&	6.58	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	892	&	Johnson	&	B	&	6.55	&	0.05	&	\citet{1978AJ.....83..606M}\\
GJ	892	&	Johnson	&	B	&	6.56	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	892	&	Johnson	&	B	&	6.58	&	0.05	&	\citet{1975MNRAS.172..667J}\\
GJ	892	&	Johnson	&	B	&	6.56	&	0.05	&	\citet{1979PASP...91..180M}\\
GJ	892	&	Johnson	&	B	&	6.57	&	0.05	&	\citet{1985A_AS...61..331O}\\
GJ	892	&	Johnson	&	B	&	6.57	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	892	&	Johnson	&	B	&	6.58	&	0.05	&	\citet{1974RMxAA...1...67M}\\
GJ	892	&	Johnson	&	B	&	6.55	&	0.05	&	\citet{1971A_A....12..442M}\\
GJ	892	&	Stromgren	&	b	&	6.14	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	892	&	Stromgren	&	b	&	6.13	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	892	&	Stromgren	&	b	&	6.13	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	892	&	Stromgren	&	b	&	6.13	&	0.08	&	\citet{1970ApJS...22..117B}\\
GJ	892	&	Stromgren	&	b	&	6.14	&	0.08	&	\citet{1990A_AS...82..531F}\\
GJ	892	&	Stromgren	&	b	&	6.14	&	0.08	&	\citet{1970AJ.....75..978C}\\
GJ	892	&	Stromgren	&	b	&	6.14	&	0.08	&	\citet{1973ApJ...179..855P}\\
GJ	892	&	Stromgren	&	b	&	6.15	&	0.08	&	\citet{1974AJ.....79.1424O}\\
GJ	892	&	Stromgren	&	b	&	6.17	&	0.08	&	\citet{1990AJ....100.1621P}\\
GJ	892	&	Geneva	&	V1	&	6.36	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	892	&	Stromgren	&	y	&	5.56	&	0.08	&	\citet{1998A_AS..129..431H}\\
GJ	892	&	Stromgren	&	y	&	5.56	&	0.08	&	\citet{1993A_AS..102...89O}\\
GJ	892	&	Stromgren	&	y	&	5.56	&	0.08	&	\citet{1983A_AS...54...55O}\\
GJ	892	&	Stromgren	&	y	&	5.56	&	0.08	&	\citet{1970ApJS...22..117B}\\
GJ	892	&	Stromgren	&	y	&	5.56	&	0.08	&	\citet{1990A_AS...82..531F}\\
GJ	892	&	Stromgren	&	y	&	5.56	&	0.08	&	\citet{1970AJ.....75..978C}\\
GJ	892	&	Stromgren	&	y	&	5.56	&	0.08	&	\citet{1973ApJ...179..855P}\\
GJ	892	&	Stromgren	&	y	&	5.56	&	0.08	&	\citet{1974AJ.....79.1424O}\\
GJ	892	&	Stromgren	&	y	&	5.56	&	0.08	&	\citet{1990AJ....100.1621P}\\
GJ	892	&	Geneva	&	V	&	5.56	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	892	&	Johnson	&	V	&	5.56	&	0.05	&	\citet{1953ApJ...117..313J}\\
GJ	892	&	Johnson	&	V	&	5.54	&	0.05	&	\citet{1967AJ.....72.1334C}\\
GJ	892	&	Johnson	&	V	&	5.56	&	0.05	&	\citet{1966ZA.....64..269A}\\
GJ	892	&	Johnson	&	V	&	5.57	&	0.05	&	\citet{1983A_AS...52..131O}\\
GJ	892	&	Johnson	&	V	&	5.56	&	0.05	&	\citet{1952ApJ...116..251S}\\
GJ	892	&	Johnson	&	V	&	5.57	&	0.05	&	\citet{1954ApJ...120..196J}\\
GJ	892	&	Johnson	&	V	&	5.62	&	0.05	&	\citet{1963ArA.....3..273O}\\
GJ	892	&	Johnson	&	V	&	5.61	&	0.05	&	\citet{1957IzKry..17...42N}\\
GJ	892	&	Johnson	&	V	&	5.56	&	0.05	&	\citet{1966MNRAS.133..475A}\\
GJ	892	&	Johnson	&	V	&	5.54	&	0.05	&	\citet{1960BAN....15..199O}\\
GJ	892	&	Johnson	&	V	&	5.56	&	0.05	&	\citet{1984A_AS...57..357O}\\
GJ	892	&	Johnson	&	V	&	5.57	&	0.05	&	\citet{1985A_AS...59..461O}\\
GJ	892	&	Johnson	&	V	&	5.57	&	0.05	&	\citet{1986A_AS...65..405O}\\
GJ	892	&	Johnson	&	V	&	5.57	&	0.05	&	\citet{1964BOTT....3..305J}\\
GJ	892	&	Johnson	&	V	&	5.57	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	892	&	Johnson	&	V	&	5.56	&	0.05	&	\citet{1978AJ.....83..606M}\\
GJ	892	&	Johnson	&	V	&	5.56	&	0.05	&	\citet{1986EgUBV........0M}\\
GJ	892	&	Johnson	&	V	&	5.56	&	0.05	&	\citet{1975MNRAS.172..667J}\\
GJ	892	&	Johnson	&	V	&	5.57	&	0.05	&	\citet{1979PASP...91..180M}\\
GJ	892	&	Johnson	&	V	&	5.58	&	0.05	&	\citet{1985A_AS...61..331O}\\
GJ	892	&	Johnson	&	V	&	5.57	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	892	&	Johnson	&	V	&	5.59	&	0.05	&	\citet{1974RMxAA...1...67M}\\
GJ	892	&	Johnson	&	V	&	5.56	&	0.05	&	\citet{1971A_A....12..442M}\\
GJ	892	&	Geneva	&	G	&	6.49	&	0.08	&	\citet{1976A_AS...26..275R}\\
GJ	892	&	1250	&	250	&	3.86	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	892	&	1250	&	250	&	3.87	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	892	&	1250	&	250	&	3.86	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	892	&	1250	&	250	&	3.8	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	892	&	1250	&	250	&	3.86	&	0.05	&	\citet{1975A_AS...22....1V}\\
GJ	892	&	2Mass	&	J	&	3.98	&	0.26	&	\citet{2003tmc..book.....C}\\
GJ	892	&	Johnson	&	J	&	3.86	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	892	&	Johnson	&	J	&	3.87	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	892	&	Johnson	&	J	&	3.8	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	892	&	1650	&	330	&	3.4	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	892	&	1650	&	330	&	3.13	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	892	&	1650	&	330	&	3.27	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	892	&	1650	&	330	&	3.4	&	0.05	&	\citet{1975A_AS...22....1V}\\
GJ	892	&	2Mass	&	H	&	3.47	&	0.23	&	\citet{2003tmc..book.....C}\\
GJ	892	&	Johnson	&	H	&	3.4	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	892	&	Johnson	&	H	&	3.27	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	892	&	2Mass	&	Ks	&	3.26	&	0.3	&	\citet{2003tmc..book.....C}\\
GJ	892	&	2200	&	440	&	3.28	&	0.05	&	\citet{1965ApJ...141..170J}\\
GJ	892	&	2200	&	440	&	3.27	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	892	&	2200	&	440	&	3.23	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	892	&	2200	&	440	&	3.27	&	0.05	&	\citet{1975A_AS...22....1V}\\
GJ	892	&	2200	&	440	&	3.18	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	892	&	Johnson	&	K	&	3.23	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	892	&	Johnson	&	K	&	3.27	&	0.05	&	\citet{1966CoLPL...4...99J}\\
GJ	892	&	Johnson	&	K	&	3.18	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
GJ	892	&	3500	&	700	&	3.17	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	892	&	3500	&	700	&	3.18	&	0.05	&	\citet{1975A_AS...22....1V}\\
GJ	892	&	Johnson	&	L	&	3.17	&	0.05	&	\citet{1968ApJ...152..465J}\\
GJ	892	&	Johnson	&	L	&	3.13	&	0.05	&	\citet{1975MNRAS.171P..19G}\\
											
\enddata											
\tablecomments{The collections of photometry used in the SED fitting routine for all objects. Refer to Section~\ref{sec:stellar_diameters} for details.}											
											
\end{deluxetable}											
											
											
											
%\bibliography{table-references}											
											
											
%\end{document}											
											
%%											
%% End of file `table.tex'.											

